Report-Sensitive Spot-Checking in Peer-Grading Systems

Peer grading systems make large courses more scalable, provide students with faster and more detailed feedback, and help students to learn by thinking critically about the work of others. A key obstacle to the broader adoption of peer grading systems is motivating students to provide accurate grades. The literature has explored many different approaches to incentivizing accurate grading (which we survey in detail), but the strongest incentive guarantees have been offered by mechanisms that compare peer grades to trusted TA grades with a fixed probability. In this work, we show that less TA work is required when these probabilities are allowed to depend on the grades that students report. We prove this result in a model with two possible grades, arbitrary numbers of agents, no requirement that students grade multiple assignments, arbitrary but homogeneous noisy observation of the ground truth which students can pay a fixed cost to observe, and the possibility of misreporting grades before or after observing this signal. We give necessary and sufficient conditions for our new mechanism's feasibility, prove its optimality under these assumptions, and characterize its improvement over the previous state of the art both analytically and empirically. Finally, we relax our homogeneity assumption, allowing each student and TA to observe the ground truth according to a different noise model.

==> 2020-AAMAS_ Peer grading (arxiv)/abstract.tex <==
\begin{abstract}
Peer grading systems make large courses more scalable, provide students with faster and more detailed feedback, and help students to learn by thinking critically about the work of others.  A key obstacle to the broader adoption of peer grading systems is motivating students to provide accurate grades.  The literature has explored many different approaches to incentivizing accurate grading (which we survey in detail), but the strongest incentive guarantees have been offered by mechanisms that compare peer grades to trusted TA grades with a fixed probability.  In this work, we show that less TA work is required when these probabilities are allowed to depend on the grades that students report. We prove this result in a model with two possible grades, arbitrary numbers of agents, no requirement that students grade multiple assignments, arbitrary but homogeneous noisy observation of the ground truth which students can pay a fixed cost to observe, and the possibility of misreporting grades before or after observing this signal. We give necessary and sufficient conditions for our new mechanism's feasibility, prove its optimality under these assumptions, and characterize its improvement over the previous state of the art both analytically and empirically. Finally, we relax our homogeneity assumption, allowing each student and TA to observe the ground truth according to a different noise model. %We also show, surprisingly, that TA workload is reduced by choosing not to spot check some students even when TA assessments are available. Finally, we test the performance of our mechanism numerically and show that it can obtain significant improvements over the fixed-probability mechanism.
%sometimes if we do not compare student reports to TA grades even when TA grades are available, the TA workload needed to incentivize students is reduced.


%Peer grading has many advantages: making large courses more scalable; providing students with faster and more detailed feedback; and helping students to learn by thinking critically about the work of others. A key strategy for motivating students to provide accurate grades is \emph{spot-checking.} Previous work has considered mechanisms that spot check each submission with a fixed probability. Here, for the first time, we show that the same incentives can be provided at lower cost by spot checking students based on the grades they report. We show that our proposed mechanism outperforms the fixed-probability mechanism and indeed minimizes the required amount of spot checking.  A surprising consequence of our main theorem is that the amount of TA work needed to incentivize students can be reduced by sometimes declining to compare student reports to TA reports even when TA reports are available.


			% We consider two novel types of report sensitive spot-checking mechanisms: the first on spot-checks each assignment based the vector of reported grades, however, the second one spot-checks each individual students based her reported grade. The spot-checking probabilites are set such that each student prefers to put in the effort for grading and report their grade to the system honestly, while the required amount of spot-checking is minimized. We find the optimal spot-checking policy in both cases and show that they always 
\end{abstract}


==> 2020-AAMAS_ Peer grading (arxiv)/comparison.tex <==
Drawing on our characterization from Section~\ref{sec:optimality}, we can now compare the workloads required by the optimal DSIC ROS, RSS and RSUS mechanisms.
%each of the different mechanisms discussed in Section~\ref{sec:nonuni}.  
%
We begin by comparing the TA workload of the optimal DSIC RSS mechanism with that of the optimal DSIC ROS mechanism. 

\begin{corollary} \label{RSS saving}
When $\joint{\firstsig} > \joint{\secondsig}$ and $\joint{\secondsig\secondsig} - \joint{\firstsig\secondsig} > \frac{c}{R} $, the TA workload of the optimal DSIC ROS mechanism exceeds that of the optimal DSIC RSS mechanism by at least $ \frac{c}{R} \cdot \frac{\joint{\secondsig}}{\joint{\firstsig\firstsig}\joint{\secondsig\secondsig}-(\joint{\firstsig\secondsig})^2}.$
	%$\frac{1}{1-\trueqp{\trueq{\firstsig}}}    \frac{1-\conp{\firstsig}{\trueq{\firstsig}}}{\left((2\conp{\secondsig}{\trueq{\secondsig}}-1) \conp{\firstsig}{\trueq{\firstsig}} - \conp{\secondsig}{\trueq{\secondsig}}\right)^2} + \frac{1}{\trueqp{\trueq{\firstsig}}}    \frac{\conp{\secondsig}{\trueq{\secondsig}}}{\left((2\conp{\firstsig}{\trueq{\firstsig}}-1) \conp{\secondsig}{\trueq{\secondsig}} - \conp{\firstsig}{\trueq{\firstsig}}\right)^2} $.
	%	\hufu{As we discussed, let's simplify this and keep the complicated expressions to any discussions.}
\end{corollary}


\begin{proof}  
By Theorem~\ref{uniform optimal}, the optimal DSIC ROS solution is $\frac{c}{R} \cdot \frac{1}{\joint{\secondsig \secondsig}-\joint{\firstsig \secondsig}}$. Let $\Vec{\firstsig}$ be a vector of length $n$ where all signals are $\firstsig$. By~\eqref{long-opt1}, this vector is be spot checked with probability $\spotcheckp{\firstsig}{n}$. By~\eqref{long-opt1} and ~\eqref{long-opt2},  $\spotcheckp{\secondsig}{k} > \spotcheckp{\firstsig}{k}$ for any $k \in \{0,\dots,n-1\}$ (recall that $\spotcheckp{\secondsig}{n}= \spotcheckp{\firstsig}{0} =0$). Therefore, $\max\{\spotcheckp{\firstsig}{j}, \spotcheckp{\secondsig}{j}\}= \spotcheckp{\secondsig}{j}$ for any vector other than $\Vec{\firstsig}$. Hence, the TA workload saved by the RSS mechanism is:

	\begin{align} 
	&	 \left(\joint{\Vec{\firstsig}} \left(\spotcheckpx^* - \frac{c}{R} \cdot \frac{ \joint{\secondsig}}{\joint{\firstsig \firstsig}\joint{\secondsig \secondsig}-(\joint{\firstsig \secondsig})^2} \right) \right. \label{Rss-saving}\\
	&\left.  + \left(1- \joint{\Vec{\firstsig}} \right) \left(\spotcheckpx^* - \frac{c}{R} \cdot \frac{ \joint{\firstsig}}{\joint{\firstsig \firstsig}\joint{\secondsig \secondsig}-(\joint{\firstsig \secondsig})^2} \right) \right)   \nonumber\\
	&\geq \frac{c}{R} \cdot \left( \frac{1}{\joint{\secondsig \secondsig}-\joint{\firstsig \secondsig}} -  \frac{ \joint{\firstsig}}{\joint{\firstsig \firstsig}\joint{\secondsig \secondsig}-(\joint{\firstsig \secondsig})^2} \right)  \nonumber\\
%	&= \frac{c}{R} \cdot \left( \frac{1}{\joint{\secondsig \secondsig}-\joint{\firstsig \secondsig}}-  \frac{\joint{\firstsig}}{\joint{\firstsig \firstsig}\joint{\secondsig \secondsig}-(\joint{\firstsig \secondsig})^2} \right) \nonumber\\
	&\geq  \frac{c}{R} \cdot \frac{\joint{\secondsig}}{\joint{\firstsig \firstsig}\joint{\secondsig \secondsig}-(\joint{\firstsig \secondsig})^2}, \nonumber
	% \\ &= c \left( \frac{\sum_{q} \trueqp{q}  \conp{\secondsig}{q}}{(\sum_{q } \trueqp{q}  (\conp{\firstsig}{q})^2)(\sum_{q} \trueqp{q}  (\conp{\secondsig}{q})^2)- (\sum_{q} \trueqp{q}  \conp{\firstsig}{q}\conp{\secondsig}{q})^2}    \right),
    	\end{align}
	where the first and second inequalities are due to the facts that $\joint{\firstsig} \geq \joint{\secondsig}$ and $\joint{\firstsig \firstsig} \geq \joint{\firstsig \secondsig}$.
\end{proof}




\begin{corollary} \label{RSS saving2}
	When %the ex ante probabilities of the two signals are equal, i.e., 
	$\joint{\firstsig}= \joint{\secondsig}$ and $\joint{\secondsig\secondsig} - \joint{\firstsig\secondsig} > \frac{c}{R} $, the TA workload of the optimal DSIC RSS mechanism is equal to that of the optimal DSIC ROS mechanism.
\end{corollary}


\begin{proof}	
The optimal DSIC ROS solution is $\frac{\frac{c}{R}}{\joint{\secondsig \secondsig}-\joint{\firstsig \secondsig}}$. Also, when $\joint{\firstsig}= \joint{\secondsig}$, $\joint{\firstsig}-\joint{\firstsig \secondsig}=\joint{\firstsig \firstsig}=\joint{\secondsig}-\joint{\firstsig \secondsig}=\joint{\secondsig \secondsig}$, and the spot-checking probabilities defined by~\eqref{opt1} and~\eqref{opt2} are equal. Thus, the TA workload that the RSS mechanism saves is:
	\begin{align*}
	& \frac{c}{R} \cdot \left(\frac{1}{\joint{\secondsig \secondsig}-\joint{\firstsig \secondsig}} - \frac{\joint{\secondsig}}{\joint{\firstsig \firstsig}\joint{\secondsig \secondsig}-(\joint{\firstsig \secondsig})^2}\right)  \\
	& \ = \frac{\joint{\firstsig \firstsig}\joint{\secondsig \secondsig}-(\joint{\firstsig \secondsig})^2- (\joint{\secondsig \secondsig}+\joint{\firstsig \secondsig})(\joint{\secondsig \secondsig}-\joint{\firstsig \secondsig})}{(\joint{\secondsig \secondsig}-\joint{\firstsig \secondsig})(\joint{\firstsig \firstsig}\joint{\secondsig \secondsig}-(\joint{\firstsig \secondsig})^2)} = 0.
	\end{align*}
	% \end{proofnoqed}
	% \begin{corollary} 
	% 	%$c(\frac{\joint{\secondsig}}{\joint{\firstsig \firstsig}\joint{\secondsig \secondsig}-(\joint{\firstsig \secondsig})^2})$.
	% \end{corollary}
	% \begin{proof}
\end{proof}


%\hufu{We may also give two expressions in the statement of the corollary.  One easier to read, the other to facilitate this discussion.} From Corollary~\ref{RSS saving}, we see that if $\conp{\firstsig}{\trueq{\firstsig}}$ or $\conp{\secondsig}{\trueq{\secondsig}}$ increase, the TA workload saved by the optimal DSIC RSS over the optimal DSIC ROS mechanism decreases.  In this sense, the RSS mechanism saves less TA workload when
% there is less noise in the system.
%the signals are less noisy in revealing the assignment quality.

%While the comparison between ROS and RSS mechanisms is a straightforward consequence of our characterization, the next comparison, our second nontrivial main result, requires more involved analysis. 
We now turn to comparing RSUS and RSS mechanisms. Because RSUS mechanisms are special cases of RSS mechanisms, it is obvious that the former perform weakly worse than the latter, all else being equal. Our second nontrivial main result shows something stronger: that the optimal RSS mechanism is {strictly} better than all RSUS mechanisms, even when the latter are strengthened by being required to satisfy only the ICCP solution concept.  The proof is based on a linear program that lower bounds the workload of the optimal RSUS mechanism under the ICCP constraints. We show that this workload is still greater than that of the optimal RSS mechanism. Recall that RSUS mechanisms spot check all students whenever the TA is consulted.  Our result thus implies that the TA workload can be decreased by choosing not to spot check certain students even when the TA spot checks other students.

% either the optimal DSIC ROS mechanism or the optimal RSUS mechanism. 
% This is true even when give an advantage to RSUS mechanisms by allowing them to operate under the weaker ICCP solution concept.
\begin{theorem}
	\label{thm:RSS-RSUS}
	%\hufu{The statement is clearly not right given the corollary above.  When $P_{\firstsig} = P_{\secondsig}$, everything collapses to the same, and there is no strict saving.}
	When $\joint{\firstsig} > \joint{\secondsig}$ and $\sigcond{\firstsig}{\firstsig} - \joint{\firstsig} \geq \frac{c}{R} $, the optimal RSS under the DSIC solution concept spot checks strictly less than the optimal RSUS mechanism under the ICCP solution concept.
\end{theorem}

\textit{Remark:}	It is straightforward to see that in the case of $\joint{\firstsig} = \joint{\secondsig}$, the TA workload of the optimal ICCP RSUS mechanism is equal to the optimal DSIC RSS and ROS mechanisms.


\begin{proof}
	The RSUS mechanisms are special cases of the RSS mechanisms, where $\spotcheckp{\firstsig}{k}=\spotcheckp{\secondsig}{k}= \spotcheckpx(k)$ for $k \in \{0,\dots,n\}$. We prove this theorem by showing that the optimal solution of an adapted version of the RSS convex optimization problem for the RSUS mechanisms is strictly worse than the optimal DSIC RSS solution defined by~\eqref{opt1} and \eqref{opt2}. Once  $\spotcheckp{\firstsig}{k}=\spotcheckp{\secondsig}{k}$, for any student $i$, we get that %\footnote{Abusing notation, we assume that $\spotcheckpx(k)$ has only one dimension here.}
	\begin{multline}
	\min_{\substack{\spotcheckpx}}    \sum_{t \in Q} \trueqp{t} \sum_{j = 0}^n \binom{n}{j} (\conp{\firstsig}{t})^j\\ \cdot (\conp{\secondsig}{t})^{n - j} \spotcheckpx(k) \label{obj00} 
	\end{multline}
	subject to:	
%	\begin{align}
%	& \Ex[s_i]{   \Ex[\sigta \sim \conp{\sig}{s_i}]{Y(s_i, \sigta)} \spotcheckpx_{k+\mathbb{1}_{s_i=a}}}  \label{firstgroup0} \\
%	&- \Ex[\sigta \sim \joint{\sig}]{Y(a, \sigta)}  \spotcheckpx_{k+1} \geq c, \ \forall k \in \{0,\dots,n-1\}    \nonumber \\
%	& \Ex[s_i]{   \Ex[\sigta \sim \conp{\sig}{s_i}]{Y(s_i, \sigta)} \spotcheckpx_{k+\mathbb{1}_{s_i=a}}} \label{firstgroup10} \\
%	& -  \Ex[\sigta \sim \joint{\sig}]{Y(b, \sigta)} \spotcheckpx(k) \geq c, \ \forall k \in \{0,\dots,n-1\}   \nonumber \\
%	&   \Ex[\sigta \sim \conp{\sig}{s_i=a}]{Y(a, \sigta)}  \spotcheckpx_{k+1} \label{second group0}\\
%	& \ \geq   \Ex[\sigta \sim \conp{\sig}{s_i=a}]{Y(b, \sigta)} \spotcheckpx(k), \ \forall k \in \{0,\dots,n-1\} \nonumber \\
%	&    \Ex[\sigta \sim \conp{\sig}{s_i=b}]{Y(b, \sigta)} \spotcheckpx(k) \label{second group10}\\
%	& \  \geq  \Ex[\sigta \sim \conp{\sig}{s_i=b}]{Y(a, \sigta)}  \spotcheckpx_{k+1}, \ \forall k \in \{0,\dots,n-1\} \nonumber \\
%	& 0 \leq \spotcheckpx_k \leq 1. \  \forall k \in \{0,\dots,n\}  \label{third group0}
%	\end{align}	
    \begin{align}
 	   - &  {\joint{\firstsig \secondsig}}     \spotcheckpx(k+1) + {\joint{\secondsig \secondsig}}    \spotcheckpx(k)  \geq \frac{c}{R} \ \  \forall k \in \{0,\dots, n-1\}  \label{120} \\
	     & {\joint{\firstsig \firstsig}}     \spotcheckpx(k+1) - {\joint{\firstsig \secondsig}}    \spotcheckpx(k)  \geq \frac{c}{R}    \ \ \forall k \in \{0,\dots, n-1\} \label{121} \\
	    - & {\joint{\firstsig \secondsig}}     \spotcheckpx(k+1) + {\joint{\secondsig \secondsig}}    \spotcheckpx(k)  \geq 0 \ \ \forall k \in \{0,\dots, n-1\}  \label{1200} \\
	     & {\joint{\firstsig \firstsig}}     \spotcheckpx(k+1) - {\joint{\firstsig \secondsig}}    \spotcheckpx(k)  \geq 0   \ \ \forall k \in \{0,\dots, n-1\} \label{1211} \\
	   & 0 \leq \spotcheckpx(k) \leq 1 \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \forall k \in \{0,\dots,n\}
    \end{align} 
	The derivation of Constraints~\eqref{120}--\eqref{1211} is similar to that of Constraints\eqref{eq:ica-lazy-opponents-simplified}--\eqref{eq:misreport-a-b-simplified} in the proof of Theorem~\ref{main}. Observe that our optimization problem is now a linear program and that Constraints~\eqref{1200} and~\eqref{1211} are implied by Constraints~\eqref{120} and~\eqref{121}; thus, they can be removed without changing the optimal solution. 

	We start from the optimal DSIC ROS solution $\spotcheckpx^*$ and decrease  $\spotcheckpx(n)$ by $\dif{\spotcheckpx(n)}=  \frac{c}{R} \cdot  \frac{{\joint{\firstsig}}-{\joint{\secondsig}}}{{\joint{\secondsig \secondsig}}-{\joint{\firstsig \secondsig}}}  \cdot  \frac{{\joint{\secondsig \secondsig}}}{{\joint{\firstsig \firstsig}}{\joint{\secondsig \secondsig}}-(\joint{\firstsig \secondsig})^2}$ and the rest of the spot checking probabilities by
	\begin{eqnarray} \label{rate}
	\dif{\spotcheckpx(k)} = \left(\frac{{\joint{\secondsig \secondsig}}}{{\joint{\firstsig \secondsig}}}\right)      \dif{\spotcheckpx(k-1)}, \ \ \forall k \in \{0,\dots,n\}. \label{rate1}
	\end{eqnarray} 
	At $\spotcheckpx^*$, Constraint \eqref{120} becomes tight, following directly from our construction of the step size given by \eqref{rate1}. Constraint \eqref{121} is tight when $k=n-1$; the rest of the constraints are easily satisfied. Hence, we only need to show that Constraint \eqref{121} will not be violated by the specified decrease in the decision variables. 
	However, by~\eqref{rate1} we get that for $k \in \{0,\dots,n-1\}$, the ratios by which the gap between the left and right hand sides of Constraints~\eqref{121} decreases is $\left(\frac{{\joint{\firstsig \secondsig}}}{{\joint{\secondsig \secondsig}}}\right)^{(n-k)} \leq 1$  times the ratio by which the gap for the constraint corresponding to $n=k-1$ is decreasing. Therefore, the constraint corresponding to $n=k-1$ binds faster. 
	
	%Once Constraints~\eqref{120}, and~\eqref{121} for $k=n-1$ become tight, any feasible local changes to the decision variables would only increase the objective value. This is because at the obtained solution, based on the constraints structure, the only possible change to $\spotcheckpx_n$ and $\spotcheckpx_{n-1}$ which would not result in violating these constraints is to increase them together.
	
	As a result, since Constraint \eqref{120} and \eqref{121} when $k=n-1$ are all binding, we can not decrease any of the decision variables anymore without increasing another. Since every objective coefficient is positive, increasing $\spotcheckpx(k)$ for any $k \in \{0,\dots,n\}$ could be beneficial only if it resulted in decreasing the value of the rest of the decision variables, achieving an overall objective function improvement. However, if $\spotcheckpx(k+1)$ is increased then $\spotcheckpx(k)$ needs to increase as well to preserve feasibility; if $\spotcheckpx(k)$ increases then $\spotcheckpx(k-1)$ needs to increase as well; and so on. Thus, overall, there exist no local, objective-improving changes to the current values of $\spotcheckpx(k)$, and so we have identified an optimal solution to our linear program. Finding the intersection point of the binding constraints shows that $x(n)=\spotcheckpx_{\firstsig}(k) \leq x(n-1)=\spotcheckpx_{\secondsig}(k) < x(n-2),\dots, < x(0)$, where $\spotcheckpx_{\firstsig}(k)$ and $\spotcheckpx_{\secondsig}(k)$ are defined by~\eqref{opt1} and \eqref{opt2} for any $k \in \{0,\dots,n\}$. This leads to the result of the theorem statement.\footnote{Note that we actually prove more than claimed in the theorem statement: our result holds not only for the ICCP solution concept, but also for all strategies in which no students invest  grading effort.}
\end{proof}


%\hufu{Unclear to me that this paragraph belong here. KLB: I don't feel strongly; we could cut it. I put it here because it's a statement about comparing mechanisms, which is what the section is about. It can't go in the intro because we don't there discuss RSS, ROS etc.}
%Gao et al \cite{gao2016incentivizing} showed that a given family of peer-prediction-based mechanisms require strictly more spot checking than the optimal DSIC ROS mechanism, even while providing weaker incentives for truthful reporting. It therefore follows from our results that the optimal RSS mechanism similarly outperforms peer-prediction-based mechanisms.



==> 2020-AAMAS_ Peer grading (arxiv)/conclusion.tex <==
% \section{Conclusion} 
% \label{sec:conclusion}

%It is worth mentioning that there is stronger solution concept that can be considered in peer grading, which is to let the student consider those students who might change their signal after observing.	





We have investigated peer grading mechanisms that achieve dominant strategy incentive compatibility by using TAs to spot check students, and have focused on minimizing the required TA workload. We have explored mechanisms for \emph{report-sensitive spot checking}: varying spot-checking probabilities based on the profile of grades that all students report for a given assignment. We proposed a simple optimal DSIC ``PRSS'' mechanism, and showed that it minimizes the required spot-checking budget (across both the ``RSS'' mechanisms and the more constrained ``RSUS'' mechanisms even under a weaker solution concept) and outperforms the (``ROS'') mechanisms that spot checks all students with a fixed, report-oblivious probability. We evaluated the performance of the optimal DSIC RSS mechanism both analytically and empirically.  Finally, we extended our results to a setting which allowed each student and TA to observe the ground truth according to a different noise model.

We consider the most important direction for future work to be generalizing our results beyond two signals. We note that this would require a fundamentally different proof technique, as our convex programming formulation depends critically on the problem's two-signal structure. We expect that the multi-signal setting would also require other variations in the model. Notably, in such domains it becomes natural to impose an ordering over the signals and to reward agents according to the distance between their reports and that of the TA, rather than rewarding all ``correct'' reports equally.
%
Another limitation of our work is the assumption that the prior distribution over signals is known to the mechanism designer. The derivation of prior-independent report-sensitive mechanisms is a second, worthwhile direction for future work. One possible strategy for building such mechanisms could be learning the prior in a repeated setting.



==> 2020-AAMAS_ Peer grading (arxiv)/hetero.tex <==
So far, our analysis has been limited to a model in which students' and TA's signals are drawn from the same signal distribution. 
% for two main reasons. First, we wanted to compare the optimal DSIC RSS mechanism to the optimal DSIC ROS mechanism and this comparison is only interesting when mechanisms do not differentiate between students. Second, we wanted to keep our analysis and notation simple and easier to follow. 
In this section, we show that our main structural result, % extend our optimally result in 
Theorem~$\ref{main}$, in fact extends to a model in which students' and TA's signals are from different distributions. 

More formally, suppose each student~$i$, by exerting effort at cost $c_i$, can examine the submission and observe a signal~$s_i \in Q$; conditioning on the submission's quality~$q$, each signal $\sig_i$ is drawn independently from a commonly known distribution~$\Prx{\sig_i|q}$. 
Also, the TA's signal~$\sigta$ is independently drawn from distribution $\Prx{\sigta|q}$.
%independently from the students' signals.
Note that the key difference from the setting in the first few sections is that $\Prx{\sig_i | q}$ and $\Prx{\sigta|q}$ may all be different from each other.  %We refer to this as the \emph{heterogeneous} setting.

Let $\Vec{r}_{-i}$ be the vector of reports made by all students except~$i$; 
$\spotcheckpx^{\firstsig}_i(\vec r_{-i})$ %: Q^{n-1} \rightarrow[0,1]$ 
denote the probability of spot checking student~$i$ when she reports $\firstsig$, while the other students report~$\vec r_{-i}$; 
% $\spotcheckpx^{\firstsig}_i (\Vec{r}_{-i})$ takes a vector of reports $\Vec{r}_{-i}$ as input and returns the probability that the mechanism will spot check agent $i$ reporting $\firstsig$. 
similarly, $\spotcheckpx^{\secondsig}_i(\vec r_{-i})$ denotes the probability of spot checking student~$i$ when she reports~$\secondsig$.
%: Q^{n-1} \rightarrow[0,1]$ be an analogous function for computing the probability of spot checking agent $i$ for reporting $\secondsig$. 
% The following theorem characterizes the optimal DSIC report-sensitive spot-checking mechanism for the heterogeneous case:
\begin{theorem} \label{main1}
	\label{thm:opt-RSS1}
	If for any student $i$ and signal $\sig_i \in Q$, % and any $c_i,R > 0$, 
	\begin{align*}
	    \min_{l \in Q} \{\Prx{\sig_i=l \given \sigta = l} - \Prx{\sig_i =l}\} \geq \frac{c_i}{R}, 
	\end{align*}
	the PRSS mechanism with the following spot-checking probabilities is DSIC and minimizes the TA workload among all DSIC spot-checking mechanisms:
	\begin{align}
	\spotcheckpx^{\firstsig}_i (\Vec{r}_{-i}) &=  \frac{  \frac{c_i}{R} }{\Prx{\sig_i=\secondsig \given \sigta = \secondsig} - \Prx{\sig_i =\secondsig}} \ \ \ \forall \Vec{r}_{-i} \in Q^{n-1}  \label{opt11} \\
	\spotcheckpx^{\secondsig}_i (\Vec{r}_{-i}) &=  \frac{  \frac{c_i}{R}}{\Prx{\sig_i=\firstsig \given \sigta = \firstsig} - \Prx{\sig_i =\firstsig}} \ \ \ \forall  \Vec{r}_{-i} \in Q^{n-1}; \label{opt21}
	\end{align}
	if
	$\min_{l \in Q} \{\Prx{\sig_i=l \given \sigta = l} - \Prx{\sig_i =l}\} < \frac{c_i}{R} $ for any $i$ and~$l$,
	there exists no DSIC spot-checking mechanism.
	% minimize the expected amount of any RSS mechanism assuming that everyone is truthful and under the DSIC constraints.
\end{theorem}

\begin{proof} [Proof Sketch]
We first note that Eqs.~\eqref{eq:ica-lazy-opponents-simplified} and ~\eqref{eq:icb-lazy-opponents-simplified} in the proof of Theorem~\ref{main} are defined for each student $i$ and do not depend on the signal distribution of any student except student $i$. When the signal distribution for the TA and Students are different, the only change in~\eqref{eq:ica-lazy-opponents-simplified} and ~\eqref{eq:icb-lazy-opponents-simplified} is that instead having $n$ pair of such constraints and $2n$ variables, there are $2^{n-1}$ constraints and $2^n$ variables, with $\spotcheckpx^{\firstsig}_i (\Vec{r}_{-i})$ and $\spotcheckpx^{\secondsig}_i (\Vec{r}_{-i})$ as a pair for each~$\Vec{r}_{-i}$.  Let $\Vec{s}_{-i}$ be the signal observed by all students except student $i$. The objective function in minimization problem defined in the proof of Theorem~\ref{main} for minimizing the TA workload subject to \eqref{eq:ica-lazy-opponents-simplified} and~\eqref{eq:icb-lazy-opponents-simplified} can be redefined as follows: 
	\begin{multline*}
		\min_{\spotcheckpx^{\firstsig}_i, \spotcheckpx^{\secondsig}_i} \sum_{\Vec{s} \in Q^n} \sum_{t \in Q} \trueqp{t} \cdot
		 \prod_{j \in N} \Prx{s_j=l_j|q=t}  \max_{i} \{\spotcheckpx^{\sig_i}_i (\Vec{s}_{-i})\} % \label{obj0}  
	\end{multline*}
	with $0 \leq \spotcheckpx^{\firstsig}_i (\Vec{r}_{-i}), \spotcheckpx^{\secondsig}_i (\Vec{r}_{-i}) \leq 1$ for all $\Vec{r}_{-i} \in Q^{n-1}$ and $i$, 
which is again a convex function due to the presence of the $\max$ functions. Since the constraints are again linear and with the same structure, the same argument about the optimally of the intersection of the constraints can be applied here. This means that for each $\Vec{r}^{-i} \in Q^{n-1}$, the intersection of the corresponding pairs of constraints defined similar to \eqref{eq:ica-lazy-opponents-simplified} and~\eqref{eq:icb-lazy-opponents-simplified}, which are expressed by~\eqref{opt11} and~\eqref{opt21}, give optimal solution to the above optimization problem. The arguments in the Step 2 of the proof of Theorem~\ref{main} are also directly applicable here. This completes the proof. 
\end{proof}

==> 2020-AAMAS_ Peer grading (arxiv)/intro.tex <==
	% \section{Introduction}
	
Peer grading has the potential to improve educational outcomes in three main ways: (i) making classes more scalable by offloading some grading work to students, (ii) providing students with faster and more detailed feedback, and (iii) improving student learning by providing opportunities to think critically about the work of others. Various recent implementations of peer grading mechanisms make such systems relatively easy to deploy in practice \citep{wright2015mechanical,de2014crowdgrader,merrifield2009telescope}. 
%
The broader adoption of such systems faces a common, critical obstacle: motivating students to provide accurate grades. A natural solution is asking multiple students to grade the same assignment and rewarding them based on their behavior (e.g., based on the extent to which their grades agree with the grades given by other students).
Such solutions have been explored in detail in a large literature on \emph{peer prediction}, which considers how to incentivize agents to truthfully disclose unverifiable private information \citep{faltings2012eliciting,prelec2004bayesian,radanovic2014incentives,riley2014minimum,witkowski2012robust,witkowski2013dwelling,jurca2009mechanisms,kong2016putting,jurca2005enforcing,kamble2015truth,radanovic2013robust,shnayder2016informed}. \citet{miller2005eliciting} were the first to introduce peer prediction mechanisms in which truthful declarations constitute a Nash equilibrium. Unfortunately, these mechanisms (and, indeed, many others that were subsequently proposed) also give rise to uninformative equilibria in which agents do not reveal their private information; e.g., all students grading an assignment favorably regardless of its quality \citep{jurca2009mechanisms,witkowski2013dwelling,kong2016putting,shnayder2016informed,dasgupta2013crowdsourced}. Human experiments show that such strategic behavior does arise in practice~\citep{gao2014trick}.

Much subsequent work has attempted to identify peer prediction mechanisms in which either no uninformative equilibrium exists or the truthful equilibrium is always preferred by agents \citep{jurca2009mechanisms,witkowski2013dwelling,kong2016putting,shnayder2016informed}. %,dasgupta2013crowdsourced}. 
Two examples are particularly notable. First, \citet{dasgupta2013crowdsourced} considered a model in which agents make a binary decision about whether or not to invest costly effort, in the former case observing a noisy signal about the assignment's true value. Agents are paid according to a function that rewards agreement between graders on the same assignment and penalizes correlations in the grades assigned across different assignments. Under this mechanism, truthful reporting yields payoffs that exceed those of any other equilibrium for every agent. Furthermore, if the system contains a small fraction of agents (e.g., TAs) who are always truthful, the truthful equilibrium becomes unique.
 %
Second, \citet{de2016incentives} showed how to achieve unique, truthful equilibria by combining peer prediction with trusted reports in a hierarchical mechanism. 
One drawback of all such approaches is that they only achieve Nash equilibrium implementations, because agents' payoffs depend on other agents' actions, and so agents must reason about each other's behavior. In a classroom setting, where some students will almost surely fail to invest effort, stronger incentives may be required.
%

\citet{liu2018surrogate} showed that stronger incentives can be guaranteed by a peer prediction mechanism based on surrogate scoring rules, achieving ``uniform dominant strategy incentive compatibility'' in a setting where students make noisy observations about two possible grades. This result relies on there existing sufficiently many tasks per student; more critically, it also requires that students follow the same strategy for all tasks (and be entirely sure that all other students also do so), rather than making the more standard assumption that students make a separate strategic decision every time they are faced with a grading task.

Another approach for strengthening incentive guarantees relies on incorporating trusted graders (TAs) more fundamentally into the mechanism. For example, \citet{goel2019deep} proposed a second uniform dominant strategy mechanism that uses a set of ``golden tasks'' (for which the ground truth is known via an oracle) to incentivize high quality evaluation for a small set of agents. Then %assuming that agents' strategies do not change across different tasks, 
they use the reports provided on non-golden tasks by the agents in this set to incentivize high quality grading among other agents. Like the mechanism of \citet{liu2018surrogate}, this mechanism relies on (1) the existence of multiple tasks and (2) agents following the same strategy for all tasks; it further requires (3) the determination of ground truth for golden tasks before agents begin grading.

In this work, we follow a different thread of past work \citep{jurca2005enforcing,wright2015mechanical,gao2016incentivizing,wang2018optimal,goel2019deep}, obtaining (fully) dominant strategy mechanisms by guaranteeing that, with sufficiently high probability, each student report is compared to a trusted but noisy observation of ground truth (a TA grade). % (which we will call a \emph{spot check}) rather than to other student evaluations (or to the ground truth itself) with some sufficiently large probability.
%For example, in many real world scenarios such as large university classes, there are usually TAs who can grade at least a fraction of assignments. 
%
Because such ``spot checking'' is expensive (e.g., TAs need to be paid in proportion to the amount of work they do), it is natural to seek to minimize the amount of spot checking required to obtain dominant strategies. This minimization problem was first attacked by \citet{gao2016incentivizing}, who proposed a very simple mechanism that makes truthfulness a dominant strategy by unconditionally rewarding students when they are not spot checked and otherwise penalizing them to the extent that they disagree with the TA. They compared this mechanism with various alternatives based on peer prediction, showing that the latter require strictly more spot checking than the former, even despite the fact that peer-prediction-based mechanisms do not offer dominant strategies.

Gao et al's model always performs spot checks with some fixed probability. It is intuitive to think that \emph{report-sensitive spot checking}---that is, varying the spot-checking probability based on the students' reports---could lower the expected amount of spot checking required overall. For example, imagine that an instructor already knows that a given problem set is extremely difficult. If the reported grades for a given submission are all very high, the instructor might believe that there is an increased likelihood that students have reported dishonestly, and so might want to spot check with a higher probability. 
%
It turns out to be nontrivial to confirm or refute this intuition, for two key reasons. First, more complex ways of computing spot check probabilities opens the door to new ways for students to manipulate a mechanism. Second, students' interests become intertwined in a new way, since spot-checking probabilities now depend on other agents' strategies. 

Despite these obstacles, this paper (1) identifies the optimal dominant-strategy incentive-compatible (DSIC) report-sensitive spot-checking mechanism; (2) identifies necessary and sufficient conditions for such a mechanism's existence; (3) shows that the new mechanism requires less TA work on expectation than the mechanism of Gao et al; and that (4) the new mechanism exists for a broader range of parameter values. One interesting property of our new mechanism is that it sometimes chooses not to spot check students even when TA assessments are available for the assignments they graded: we show that making full use of TA assessments has the perverse effect of increasing expected workload overall.

Like much other work in the literature [e.g.,~\citealp{dasgupta2013crowdsourced},~\citealp{liu2018surrogate},~\citealp{wang2018optimal}], our analysis is limited to the case where students are asked to report only binary (positive or negative) grades about each assignment. Our new mechanism is general in several other, important senses: it allows for arbitrary numbers of graders per assignment and nearly arbitrary prior probability distributions over both the true grades and the noise models describing the probabilities that students and TAs will observe each signal given the ground truth. In the first part of the paper we assume that these noise models are homogeneous (identical across all students and TAs); in the last section, we generalize our results to the fully heterogeneous case (each agent can grade according to a different noise model).

%\subsection{Other Related Work}
	 
%

%In fact, we prove an even stronger result, that TA workload of the optimal DSIC mechanism is smaller than a mechanism which always spot checks every students in the presence of the TA assessment, even when the latter is optimal under a weaker solution concept than DSIC.  
%\subsection{Other Related Work}
	 
%

Finally, we mention two final strands of recent, related work. \citet{wang2018optimal} proposed a different approach for designing peer grading systems that also varies spot check probabilities. Their model is substantially different from ours, and hence their mechanism is not directly applicable to our setting. Like us, they study strategic students who make a binary decision about whether to invest effort; as we do in the last section of this paper, they assume that agents' noise models are heterogeneous. 
% More specifically, they assume a fixed budget for spot checking and study how to allocate this budget to maximize overall grading accuracy given strategic students who make a binary decision about whether to invest effort. 
However, they also assume that TAs can directly observe whether a student invested effort, making it simple to ensure that a spot-checked student who invested no effort gets no reward. In contrast, we assume that the TA noisily observes the assignment's grade and is only able to compare this observation with the student's own report, which is either a noisy signal or a misreport; thus, students who invest no effort cannot reliably be identified. \citet{xiao2018incentive} studied incentive mechanisms for peer reviewing in a repeated setting. In their model, students benefit from receiving high quality reviews and decide on the amount of effort to put in when reviewing others. Their proposed mechanism incentivizes high-quality reviewing by rating students' reviewing performance over time and using this rating to match highly ranked reviewers with each other. Key caveats are that the mechanism relies on the ability to accurately score reviewing quality and that high-quality reviewing is incentivized only in equilibrium.

In the following, we first define our model and  
% We talk more about the spot-checking idea in Section~\ref{spot-checking}. 
formalize the mechanisms that we study throughout the paper (Section~\ref{sec:model}). We next prove that our proposed mechanism is optimal (Section~\ref{sec:optimality}) and show that it outperforms alternatives (Section~\ref{sec:comparison}) by demonstrating a separation analytically and then quantifying the gap via numerical experiments. Finally, we extend our results to heterogeneous student and TA noise models (Section~\ref{sec:hetero}) and conclude (Section~\ref{sec:conclusion}).





==> 2020-AAMAS_ Peer grading (arxiv)/mechanisms.tex <==
% \section{The Non-uniform Spot-checking Mechanism} 
% \label{sec:nonuni}

A focus of our work is on minimizing the need for the TA's input via \emph{spot-checking mechanisms}.
A spot-checking mechanism takes in students' reported signals and decides both whether a TA signal is needed and how much to reward the students.  

% A spot-checking mechanism asks each student~$i$ to report a signal~$\reporti$, then maps the profile of reports to a probability with which the a \emph{spot-checking} is performed; when spot-checking occurs, the mechanism rewards each student~$i$ by comparing her report~$\reporti$ to the TA's signal~$\sigta$; otherwise the mechanism rewards each student by comparing her report~$\reporti$ to the other students' reports~$\reportsmi$.  Formally,

% In a spot-checking mechanism, each student is asked to report her signal. The mechanism then maps the profile of reports to a spot-checking probability and a reward to each student. 
% Our definition of the spot-checking mechanism includes the version of the definition given by \cite{gao2016incentivizing} as a special case. 
% Formally:

%Let $\Delta^k$ denote the standard $k$-simplex (the set $\left\{\theta_0 u_0 + \dots +\theta_k u_k ~\bigg|~ \sum_{i=0}^{k} \theta_i=1 \mbox{ and } \theta_i \ge 0 \mbox{ for all } i\right\}$).%; hence $\Delta^{|X|}$ is the set of probability distributions over a discrete set $X$. %Let  $\Delta^* = \bigcup_{k=1}^\infty \Delta^k$ denote the space of all finite standard simplices.

\begin{definition}[Spot-checking mechanism]
	\label{def:mech}
	A \emph{spot-checking mechanism} is defined by a tuple $(x_{\firstsig}, x_{\secondsig}, Y)$, where:
	\begin{enumerate}
	    \item $\spotcheckpx_{\firstsig}:\{0\} \cup \mathds{N}\times \mathds{N}\rightarrow[0,1]$ denotes the probability of spot checking an agent who reports $\firstsig$. Given two non negative integers $(k,n)$ specifying the number of $\firstsig$'s reported by the agents and the total number of agents, $\spotcheckpx_{\firstsig}(k,n)$ returns the probability that the mechanism will spot check each agents reporting $\firstsig$. The probability $\spotcheckpx_{\firstsig}(0,n)$ is set to zero.
	    \item $\spotcheckpx_{\secondsig}: \{0\} \cup \mathds{N}\times \mathds{N}\rightarrow[0,1]$ is an analogous function for computing the probability of spot checking an agent who reports $\secondsig$. The first argument remains the total number of agents who report $\firstsig$, not $\secondsig$. The probability $\spotcheckpx_{\secondsig}(n,n)$ is zero.
	    \item $Y: Q \times Q\rightarrow \mathds{R}^+$ denotes the reward given to a student who is spot checked. $Y(r, \sigta)$ is the reward of a spot-checked student who reported $r$ when the TA reported signal $\sigta$. When a student is not spot checked, she receives no reward.
	\end{enumerate}
	The $x$ functions are defined for every $n$ because we require peer grading mechanisms to work for any number of agents. However, when $n$ is obvious from context, we will overload notation and write simply $\spotcheckp{\firstsig}{k}$ and $\spotcheckp{\secondsig}{k}$.
\end{definition}
	
% 	$P = (\spotcheckp_0 = (\spotcheckp_0^a, \spotcheckp_0^b) = (\spotcheckp_1^a, \spotcheckp_1^b) \in [0, 1]^2, \spotcheckp_1 \in [0, 1]^2, \ldots, \spotcheckp_n \in [0, 1]^2, Y: \{a, b\}^2 \to \mathbb R_+)$.
% 	% $P=(X,Y,\vec{Z} = (Z_1, \cdots, Z_n))$, 
% 	% $P = (\spotcheckp, Y,\vec{Z} = (Z_1, \cdots, Z_n))$.   
% 	% $X: \{a,b\}^n \rightarrow [0,1]$, 
% 	At a set of student reports that contain $k$ signal~$\firstsig$'s, the mechanism spot-checks each student reporting~$\firstsig$ with probability $\spotcheckp_k^a$, and each student reporting~$\secondsig$ with probability $\spotcheckp_k^b$.  
% 	% $\spotcheckp: \{0, 1, \ldots, n\} \to [0, 1]^2$, the \emph{spot-checking function}, maps a set of student reports that contains $k$ signal~$\firstsig$'s to $\spotcheckp(k)$, also denoted as $\spotcheckp_k = (\spotcheckp_k^a, \spotcheckp_k^b)$.  A student that reports signal~$\firstsig$ will then be spot-checked with probability~$\spotcheckp_k^a$, and a student that reports signal~$\secondsig$ spot-checked with probability~$\spotcheckp_k^b$.  
% 	When student~$i$ is spot-checked, her report $r_i$ is compared with the TA's signal~$\sigta$, and is rewarded $Y(r_i, \sigta)$.  When a student is not spot-checked, she receives no reward.
% 	% report vector~$\reports = (\reporti[1], \ldots, \reporti[n])$ to a probability with which the submission is spot-checked; when spot-checking is performed, her report $r_i$ $Y: \{a,b\}^2 \rightarrow R^+$,  the \emph{spot-checking reward function}, returns the reward for each student~$i$ based on her report~$\reporti$ and the TA's signal~$\sigta$; otherwise, each $Z_i: \{a, b\}^n \rightarrow R^+$, the \emph{unspot-checked reward function}, returns the reward to student~$i$ based on $(\reporti, \reportsmi)$.
% 	% $\vec{Z} = (Z_1, \cdots, Z_n)$, $Z_i:  \{a,b\}^n \rightarrow R^+$, where each $Z_i$ is the unspot-checked reward function i.e., returns the reward that the mechanism gives to student $i$ if she is not spot-checked.
% \end{definition}

Throughout this paper we focus on mechanisms where the reward function~$Y$ is the simplest identity function: $$Y(r, \sigta) = \left \{ \begin{array}{cl} R & \text{if }r = \sigta \\ 0 & \text{otherwise,} \end{array} \right.$$
where $R \in \mathds{R}^+$
%I\!R}^+$ 
denotes the reward of matching with the TA signal. This function is called the output agreement reward function; it has been widely studied in the peer prediction literature~\citep{witkowski2013dwelling,waggoner2014output}. 
%\hufu{The two sentences that follow seem to come from nowhere and interrupt the flow.  I think they are in the wrong place, and should be justified/explained.}


% Our definition of the spot-checking mechanism includes as a special case the one in \citet{gao2016incentivizing}.  A mechanism is said to be \emph{anonymous} if $X$ is invariant under permutations of the students' identities.  Throughout the paper,  we focus on anonymous spot-checking mechanisms.
% , i.e., the mechanism does not distinguish between the students who make reports and spot-checks based on the \emph{set} of reported signals. Also,  we think of the TAs as non-strategic students, i.e., ${P_{s|q}}(.)= {P_{s_{\text{TA}}|q}}(.)$. 

% Based on our definition, when the other students report $\reportsmi$, by reporting~$\reporti$ with no effort, student~$i$'s gets utility
%A student has quasi-linear utility.  let $T_i$ be the subset of students who are investing effort to obtain a signal excluding student $i$, and $\vec{\sig}_{T_i}$ be the vector of observed signals. If we denote by $\conp{\sig}{j, \ell}$ the distribution for an independent draw of signal~$\sig$ conditioning on that $j$ independent draws in $\vec{\sig}_{T_i}$ have shown signal~$\firstsig$ and $\ell$ other independent draws have shown signal~$\secondsig$.  For student $i$, when $k$ other students report signal~$\firstsig$, among whom $j$ spent effort to examine the assignment, and $\ell$ others examined the assignment and obtain signal~$\secondsig$, the student's utility for reporting signal~$\firstsig$ without examining the assignment is 

We model students as having quasilinear utility: i.e., when investing effort and being rewarded $Y$, a student's utility is $Y - c$.  
 
 \iffalse 
 Let $T_{-i} \subseteq N \setminus \{i\}$ be the students other than $i$ who invest effort to obtain a signal, and let $\vec{\sig}_{T_{-i}}$ be the vector of signals observed by the students in $T_{-i}$.  Let us now calculate a student $i$'s expected utility for a given action.  When $k$ other students report signal~$\firstsig$, among whom only some may have spent effort to examine the assignment, $i$'s utility for reporting $\firstsig$ without examining the assignment is 
\klb{Do we want notation for this quantity (i.e., a LHS for this equation, instead of just an expression?) I think it would help, particularly showing us what is an argument and what's being marginalized over.}

\hedayat{I finally got Hu's point. I think defining the utility expressions is becoming more and more complicated, while we basically do not use it anywhere else in the paper. I am tempted to remove the utility formulations, but I feel like there should be some formalization of the utility function in this section. So, I do not know what to do with them.}


\begin{align*}
\scalebox{1}[1]{$\Ex[\vec{\sig}_{T_{-i}}]{\spotcheckp{\firstsig}{k+1} \sum_{s \in Q} \Prx{\sigta =s| \vec{s}_{T_{-i}}} Y(a, s)}$}.
\end{align*}
%\hufu{I don't think we introduced notations like $\conp{\sig}{\sig'}$.  As we defined it, in this notation $\sig'$ is a quality.  The same comment applies to the equation below.}
We need to take an expectation over $\vec{\sig}_{T_{-i}}$, despite having fixed $k$ and despite summing over possible signals the TA can receive, because the TA signal and other students' signals are not conditionally independent.

Analogously, we can write an expression for student $i$'s utility for being truthful, i.e., examining the assignment to obtain signal~$s_i$ and truthfully reporting~$s_i$, given that $k$ other students report signal $\firstsig$.
\begin{align*}
\scalebox{0.90}[1]{$ \Ex[s_i] {\Ex[\vec{s}_{T_{-i}} \given s_i] { \spotcheckp{\firstsig}{k+\mathbbm{1}_{s_i=\firstsig }} \sum_{s \in \{a,b\}} \Prx{\sigta =s| \vec{s}_{T_{-i}}, s_i} Y(s_i, s) }} -c$},
\end{align*}
where $\mathbbm{1}_{s_i=\firstsig }$ equals 1 if $s_i=\firstsig $ and 0 otherwise. 
\hufu{%The font for the indicator is not right.  Need to look up the right font.  There are more of these in other sections.  I didn't correct them so that later one can do a global replacement.  More importantly, 
These two expressions are not correct.  The fact that there are $k$ report~$\firstsig$'s tells us information about $s_{T_i}$, so the distribution of $s_{T_i}$ should be conditional and we need to make that clear.  Alternatively, we may just condition on how many students outside~$T_i$ are reporting~$\firstsig$ without checking.  If we are short on space, it's also not clear whether such calculations belong here.} \hedayat{I've updated the notation to be "mathbbm", instead of "mathbb". I have found both in the internet as indicator functions in latex. Not sure where to find the right one, if this is still not the right font. Also, the utility function is defined based on the student's point of view (not the God's point of view). Since our definition of DSCIC is also not from the God's point of view, I think this should be fine.} \hufu{The student does not know~$k$.  If he does, then the distribution of $s_{T_i}$ should be conditioned on~$k$.  Taking unconditioned expectation over $s_{T_i}$ while pretending to know~$k$ is not consistent.  Think about this: it snows tomorrow with probability $0.1$; if it snows tomorrow school will close with probability $1/2$; lunch is half the price if it doesn't snow.  What's the expected lunch price if school is closed?  If school is closed you know it snows so lunch must be full price.  You can't pretend you don't know anything about snow.}
\klb{I'm skipping this bit until the two of you converge (based on past experience, I suspect Hu is right :-)}


The student's utility for reporting signal $\secondsig$ with no effort and examining the assignment but misreporting the signal observed can be calculated similarly.

\fi 

%\hufu{I think this definition is still not right.  If lots of other students spent efforts and truthfully report~$\firstsig$, maybe I can be so certain about the quality that it doesn't make sense to spend effort.  Combining any number of truthful students and any report they may make is problematic.  The definition that was explained in the email makes sense.  The same comment applies to the next definition.}

%\hedayat{I updated the definition, another quick pass over the definision should be useful}
\begin{definition}[DSIC]
	\label{def:DSIC}
	A spot-checking mechanism is \emph{dominant strategy incentive compatible} (DSIC) if, for each student~$i$ and for any strategies that the other students choose, $i$'s expected utility-maximizing strategy is to be truthful, i.e., to invest effort to observe her signal and to report what she observes.
\end{definition}

The mechanism we will later show to be optimal is DSIC; however, we also define a weaker solution concept (`Incentive Compatible with Conscientious Plays", or ICCP), to allow us to compare our preferred mechanism to a broader set. A mechanism is ICCP if it is DSIC in a simplified strategy space in which students who observe their signals must report them honestly. In other words, ICCP does not allow for the possibility that students could misreport a signal that they invested effort to observe, but continues to allow for lazy students pretending to have observed arbitrary signals.
% This solution concept is motivated by the idea that students will reason strategically about 
%This solution concept is motivated by a classroom setting in which any student who decides to grade assignment would also report her observed signal, but not all the students are going to grade the assignment in the first place. 

\begin{definition}[ICCP]
	\label{def:ICCP}
	A spot-checking mechanism is \emph{Incentive Compatible with Conscientious Plays} (ICCP) if, for each student and for any strategy that other students choose, 
	%and for any set of signals they observe, 
	\emph{as long as each student that examines the assignment always reports the observed signal}, the truthful strategy, i.e., to invest effort to examine the assignment and report her observed signal, is expected utility maximizing.
\end{definition}
% \hufu{This definition is vague: it's unclear whether we apply the strategic restriction to the student in question; that is, when we say the ``truthful strategy is utility maximizing'', do we mean the truthful strategy is only better than the strategies with no observation or do we mean it's also better than those that make an observation but misreport the signal?  I believe we mean the latter, which is stronger.}
% \hedayat{I updated the definition to make is more clear.}

% We note that the mechanism that we will ultimately recommend in this paper is DSIC; we introduce the weaker ICCP concept only to show that our recommended mechanism outperforms alternatives.

\begin{definition}[TA workload] \label{TAworkload def}
For a DSIC or ICCP spot-checking mechanism, 
% the expected amount of spot checking is 
the \emph{TA workload} (or simply the \emph{workload}) is the probability with which the TA needs to provide a signal, assuming all students are truthful:
\begin{multline}
\sum_{t \in Q} \trueqp{t} \sum_{j = 0}^n \binom{n}{j} (\conp{\firstsig}{t})^j \\\cdot(\conp{\secondsig}{t})^{n - j} \max\{\spotcheckp{\firstsig}{j}, \spotcheckp{\secondsig}{j}\}.\label{eq:sc-amount}
\end{multline}
\end{definition}

The expression $\max\{\spotcheckp{\firstsig}{j}, \spotcheckp{\secondsig}{j}\}$ is TA workload needed to ensure that every student reporting $\firstsig$ is spot checked with probability $\spotcheckp{\firstsig}{j}$ and every student reporting $\secondsig$ is spot checked with probability~$\spotcheckp{\secondsig}{j}$. We say that a mechanism is \emph{optimal} for some class if it minimizes TA workload among all mechanisms in that class.

\subsection{ROS, RSS, and RSUS Mechanisms}
We now introduce three families of mechanisms, 
% which are the focus of our comparative study.  
% Note that, given our focus on the identity reward function, the mechanisms differ only in their spot-checking probabilities.  
beginning with one studied by \citet{gao2016incentivizing}.  
\begin{definition}[ROS Mechanism]
A \emph{Report-Oblivious Spot-checking (ROS)} mechanism spot checks every student with fixed probability~$x$, regardless of the students' reports.
\end{definition}

% It is straightforward to see that for ROS mechanisms, DSIC and ICCP collapse to the same solution concept. 



%\begin{definition}[Report Sensitive Spot-checking Mechanisms]
%\end{definition}

The focus of this paper is on \emph{report-sensitive} spot-checking.

\begin{definition}[RSS Mechanism]
A \emph{Report-Sensitive Spot-checking (RSS)} mechanism spot checks every student with probability that can depend on all the students' reports.
%probabilities $(\spotcheckp{\firstsig}{0}, \spotcheckp{\secondsig}{0}),$ $\ldots, (\spotcheckp{\firstsig}{n}, \spotcheckp{\secondsig}{n})$.
\end{definition}

%In a RSS mechanism, students are spot checked independently. Therefore, it might be the case that a subset of students are never spot checked, even though the TA signal is already available as a result of spot checking another student. However,
In a RSS mechanism, we determine whether to spot check each student independently: i.e., we sometimes refrain from spot checking one student even when the TA signal is already available from spot checking another student. This seems wasteful: once the TA spot checks one student, it costs them no additional work to use the observed signal to spot check other students too. We now define a class of mechanisms that leverages this fact.

\begin{definition}[RSUS Mechanism]
A \emph{Report-Sensitive, Uniform Spot-checking (RSUS)} mechanism ensures that whenever one student is spot checked, all are spot checked. 
\end{definition}

In RSUS mechanisms, $\forall j \in \{0, \ldots, n\}$, $\spotcheckp{\firstsig}{j} = \spotcheckp{\secondsig}{j}$; of course, it still allows for $j \neq j'$ that $\spotcheckp{\firstsig}{j} \neq \spotcheckp{\firstsig}{j'}$.
A main result of this paper is that RSUS mechanisms can require strictly larger spot-checking budgets than a DSIC RSS mechanism, and are hence strictly suboptimal, not just under the DSIC solution concept but even if they only need to satisfy the weaker ICCP solution concept.  In other words, paradoxically, in order to minimize the overall TA workload, 
% while providing correct incentives to the students, 
it is necessary to commit sometimes \emph{not} to use the TA's signal to spot check {some} students. 

%\subsection*{Assumptions}


%We now set up assumptions to ensure that the ROS mechanism is DSIC at least with checking probability~$1$; if not, the setting is ill conditioned. We make these assumptions throughout the paper, including our consideration of mechanisms other than ROS. 

%Our first assumption is that a student, upon observing a signal, expects any other grader (the TA or another student) to be strictly more likely to observe the same signal than the opposite.  This assumption is needed to ensure that students are strictly incentivized to report honestly in ROS mechanisms.

%\begin{assumption}\label{assn:spot-check-prob-1}$\forall i \in N \cup \{\text{TA}\}, j \in N$,
%	\begin{align*}
%		\Prx{s_i=\firstsig  \given  s_j=\firstsig } &> \Prx{s_i=\secondsig  \given s_j=\firstsig  }, \\ 
%		\Prx{s_i =\secondsig  \given s_j =\secondsig } &> \Prx{s_i =\firstsig  \given s_j =\secondsig }.
%	% \forall i,j \in \{1,\dots,n\} \ \& \ r \neq l \in \{a,b\} \nonumber 
%	\end{align*}
%\end{assumption}


%Assumption~\ref{assn:cost} is that a student being spot checked with probability~$1$ prefers to be truthful than to report an arbitrary signal without effort.

%\begin{assumption}\label{assn:spot-check-prob-2}
%	\label{assn:cost}  
%	For any student~$i$ and any signal $s \in Q$,
%\begin{multline*} 
%	\Prx{s_i=\firstsig  , \sigta=\firstsig } \\
%	+ \Prx{s_i=\secondsig  , \sigta =\secondsig }-c > \Prx{s_i=s },
%\end{multline*} 
%which means $ \joint{\secondsig \secondsig} -\joint{\firstsig \secondsig} > c$ and $ \joint{\firstsig \firstsig} -\joint{\firstsig \secondsig} > c$.
%\end{assumption}

%Note that given Assumption~\ref{assn:spot-check-prob-1}, Assumption~\ref{assn:spot-check-prob-2} can always be made true by increasing the reward. In effect, Assumption~\ref{assn:spot-check-prob-2} can be understood as saying that rewards are large enough to outweigh the cost of effort.









==> 2020-AAMAS_ Peer grading (arxiv)/model.tex <==
% \section{Model and Preliminaries} 
% \label{sec:prelim}

A single assignment\footnote{When multiple assignments must be peer graded, our mechanisms can simply be run in parallel.} needs to be graded by a set $N$ of students (with $|N|=n$) and has an unobservable binary quality 
% There are $n$ students, a Teaching Assistant (TA), and an assignment submission.  The submission has an unknown binary quality 
$q  \in Q= \{\trueq{\firstsig}, \trueq{\secondsig}\} $ drawn from a commonly known distribution $\Prx{q}$.  
%\hufu{Can we change the notation?  $P$ is used below to denote probabitilies for signals, not for quality.  The subscript of~$P$ is consistently a signal in the paper, not a quality.  Maybe~$\pi$?  Just another side comment: the macro for the probability is defined so that it always has to take a parameter --- this is inconvenient and doesn't make much semantic sense.  }
%We denote by $\trueqp{\trueq{a}}$ and $\trueqp{\trueq{b}}$
% $\Pr(q=t)$ 
%the probability with which $q$ is $\trueq{a}$ and $\trueq{b}$ respectively. 
% where $P_q(q=t)= \Pr(q=t)$ and is denoted by $\trueqp{t}$ for $ t \in \{\trueq{a}, \trueq{b}\}$. 
% Conditioned on the quality~$q$, 


Each student~$i$, by exerting effort at cost $c$, can examine the submission and observe a signal~$s_i \in Q$ that is informative about the assignment's quality. More formally, in a way that depends on the true quality~$q$, the signals observed by different students are independently drawn from a single, commonly known distribution $\Prx{s|q}$.
% and upon incurring a cost $c$ of grading, student $i$ observes an (conditionally) independent random signal $s_i \in \{a,b\}$ drawn from a commonly known distribution ${P_{s|q}}(.)$, where ${P_{s|q=t}}(s=k)=\Pr(s=k|q=t)$, and is denoted by $\conp{k}{t}$ for $k \in \{a,b\} $ and $t \in \{\trueq{a}, \trueq{b}\}$. 
%Without loss of generality, 
%\hufu{I'd rather spell out explicitly the two inequalities.}
%(break ties arbitrary). 
% Without loss of generality, we let the signal $k$ correspond to the true quality $\trueq{k}$, i.e., $\conp{k}{\trueq{k}} \geq \conp{k}{t} $ for $k \in \{a,b\}$ and $t \in \{\trueq{a}, \trueq{b}\} $ (break ties arbitrary). 
The \emph{ex ante signal distribution} is then
% by the total probability rule:
\begin{eqnarray*} 
	\Prx{s=l} = \sum_{t \in Q} \conp{l}{t} \trueqp{t}.
	% P_{s|q=t} (k) \cdot P_q(t). \ \ \ \ \ \ \ \forall k \in \{a,b\}
\end{eqnarray*}
%We name the grades and signals so that $\conp{k}{\trueq{k}} \geq \conp{k}{t} $ for $k \in \{a,b\}$ and $t \in \{\trueq{a}, \trueq{b}\}$, and $\joint{a} \geq \joint{b}$.


%; i.e., , for $\vec l \in Q^n$.  
We denote by $\joint{\vec l}$ the \emph{ex ante} probability of each agent receiving the signal corresponding to its index in vector~$\vec l$.
%; i.e., , for $\vec l \in Q^n$.  
By our assumption of conditional independence, this is 
\begin{align}
\joint{\vec l} :=& \Prx{s_1 = l_1, \ldots, s_n = l_n} \nonumber\\
=& \sum_{t \in Q} \trueqp{t} \prod_{j \in N} \Prx{s_j=l_j|q=t}. \label{joint}
\end{align}
Because of conditional independence, any two vectors of reports $\vec l$ and $\vec {l'}$ containing the same numbers of $\firstsig$'s and $\secondsig$'s occur with the same probability: $\joint{\vec l} = \joint{\vec l'}$.  For this reason, we often drop the ordering in the subscript, writing, e.g., $\joint{(\firstsig, \secondsig)} = \joint{(\secondsig, \firstsig)} = \joint{\firstsig \secondsig}$, and similarly for longer vectors. We name the signals so that $\joint{\firstsig} \geq \joint{\secondsig}$ (note that this implies $\joint{\firstsig}- \joint{\firstsig\secondsig}= \joint{\firstsig \firstsig} > \joint{\secondsig \secondsig} = \joint{\secondsig}- \joint{\firstsig\secondsig}$). We also denote by $\sigcond{l}{t}$, the probability that an agent observes signal $l \in Q$ conditioned on another agent observing signal $t \in Q$. 
% We denote the ex ante joint signal distribution $P_{\vec s}(\vec{s}=\vec{k}) = \Pr(\vec{s}=\vec{k}) $ by $\joint{\vec{k}}$ for $\vec{k} \in \{a,b\}^n$.
% and $h \in N$. 
% Without loss of generality, 

Besides the students, a teaching assistant (TA) may also receive a signal. Formally,  signal~$\sigta$ is drawn from $\Prx{s|q}$ independently from the students' signals. % and again depends on the assignment's quality~$q$.



\paragraph{Strategy space} 
% In our model, 
In our model, each student faces two strategic choices: whether to expend effort grading the assignment and what grade to report.  Three actions are thus possible: the student (i) may be \emph{truthful}, investing effort to examine the assignment, observing her signal, and reporting this signal; (ii) may invest effort but report a different signal than the one she observed; or (iii) may choose not to invest effort and report an arbitrary signal.  In contrast, the TA is not a strategic agent.  When asked to grade the assignment, the TA always reports an independently observed signal.  
% 's strategy is to choose from (i) not to put in the grading effort and report an arbitrary signal, (ii) to grade the submission but report a signal different from her observation, or (iii) to be \emph{truthful}, i.e, to grade the submission and report her observed signal. Also, each student~$i$ has quasi-linear utility







==> 2020-AAMAS_ Peer grading (arxiv)/notation.tex <==
%% General machinery
\newcommand{\AutoAdjust}[3]{\mathchoice{ \left #1 #2  \right #3}{#1 #2 #3}{#1 #2 #3}{#1 #2 #3} }
\newcommand{\Xcomment}[1]{{}}
\newcommand{\eval}[1]{\left.#1\vphantom{\big|}\right|}
\newcommand{\inteval}[1]{\Big[#1\Big]}
\newcommand{\InParentheses}[1]{\AutoAdjust{(}{#1}{)}}
\newcommand{\InBrackets}[1]{\AutoAdjust{[}{#1}{]}}% {\left[{#1}\right]}
\newcommand{\Ex}[2][]{\operatorname{E}_{#1}\InBrackets{#2}}
\newcommand{\Prx}[2][]{\operatorname{Pr}_{#1}\InBrackets{#2}}
\def\prob{\Prx}
\def\expect{\Ex}
\newcommand{\dd}{\mathrm{d}}  % for integrals
\newcommand{\given}{\;\mid\;}
\newcommand{\eps}{\epsilon}




\newcommand{\noaccents}[1]{#1}
\newcommand{\newagentvar}[3][\noaccents]{%
\expandafter\newcommand\expandafter{\csname #2\endcsname}{#1{#3}}%
\expandafter\newcommand\expandafter{\csname #2s\endcsname}{#1{\boldsymbol{#3}}}%
\expandafter\newcommand\expandafter{\csname #2smi\endcsname}[1][i]{#1{\boldsymbol{#3}}_{-##1}}%
\expandafter\newcommand\expandafter{\csname #2i\endcsname}[1][i]{#1{#3}_{##1}}%
\expandafter\newcommand\expandafter{\csname #2ith\endcsname}[1][i]{#1{#3}_{(##1)}}%
}

\newagentvar{sig}{s}
\newagentvar{report}{r}
\newcommand{\sigta}{\sig_{\mathrm{TA}}}
\newcommand{\firstsig}{a}
\newcommand{\secondsig}{b}


\newcommand{\q}[1]{``#1''}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\joint}[1]{P_{#1}}
\newcommand{\jointa}[2]{\Prx{\sigta=#1,\sig_i= #2}}
\newcommand{\jointb}[2]{\Prx{\sigta=#1,\sig_i= #2}}
\newcommand{\sigcond}[2]{P_{#1|#2}}
\newcommand{\trueqp}[1]{\Prx{q=#1}}
\newcommand{\conp}[2]{\Prx{\sig_i=#1|q=#2}}
\newcommand{\conpm}[4]{\Prx{#1=#2|#3=#4}}
\newcommand{\trueq}[1]{#1}
% \newcommand{\spotcheckp}[2]{x_{#1}^{#2}}
\newcommand{\spotcheckp}[2]{x_{#1}(#2)}
\newcommand{\spotcheckpx}{x}
\newcommand{\dif}[1]{\bigtriangleup #1}

\makeatletter
\newenvironment{proofnoqed}[1][\proofname]{\par
	\normalfont \topsep6\p@\@plus6\p@\relax
	\trivlist
	\item[\@proofindent\hskip\labelsep
	{\@proofnamefont #1\@addpunct{.}}]\ignorespaces
}{%
	\endtrivlist\@endpefalse
}
\makeatother



























	
	\iffalse
	In the following, we prove a useful lemma about the joint signal distribution that will be used in the analysis later in the paper.
	
	\begin{lemma}
		Under the assumption defined by \eqref{existanceoftruthful} and the conditional independence assumption, if $\conp{k}{\tureq{k}} \geq 1/2$ for $k \in \{a,b\}$, the signal joint distribution satisfies the following conditions:
		\begin{eqnarray} \label{property}
		{\joint{bbb} \cdot  {{\joint{ab}}} &\geq  {{\joint{abb}}} \cdot  {{\joint{bb}}} \label{property1}
		\end{eqnarray}
	\end{lemma} 
	
	
	\begin{proof}
		By the conditional independence assumption, we can write: 
		\begin{equation*}
		\begin{split}
		({p^3_{b|\trueq{a}}}  {p_{\trueq{a}}}+{p^3_{b|\trueq{b}}}  {p_{\trueq{b}}} )
		\cdot  ({p_{a|\trueq{a}}} {p_{b|\trueq{a}}}  {p_{\trueq{a}}}+ {p_{a|\trueq{b}}} {p_{b|\trueq{b}}} {p_{\trueq{b}}}   ) 
		\geq ({p_{a|\trueq{a}}} {p^2_{b|\trueq{a}}} {p_{\trueq{a}}} + {p_{a|\trueq{b}}} {p^2_{b|\trueq{b}}} {p_{\trueq{b}}})
		\cdot ({p^2_{b|\trueq{a}}} {p_{\trueq{a}}} + {p^2_{b|\trueq{b}}} {p_{\trueq{b}}} )
		\end{split}
		\end{equation*}
		after doing the multiplications we get:
		\begin{eqnarray*}
			{p^4_{b|\trueq{a}}} {p_{a|\trueq{a}}} {p^2_{\trueq{a}}} + {p_{a|\trueq{b}}} {p^4_{b|\trueq{b}}} {p^2_{\trueq{b}}}  
			+ {p_{\trueq{a}}}{p_{\trueq{b}}} {p_{b|\trueq{b}}} {p_{a|\trueq{b}}} {p^3_{b|\trueq{a}}} +  {p_{\trueq{a}}}{p_{\trueq{b}}} {p_{b|\trueq{a}}} {p_{a|\trueq{a}}} {p^3_{b|\trueq{b}}} \\
			\geq {p^4_{b|\trueq{a}}} {p_{a|\trueq{a}}} {p^2_{\trueq{a}}} + {p_{a|\trueq{b}}} {p^4_{b|\trueq{b}}} {p^2_{\trueq{b}}} 
			+ {p_{\trueq{a}}}{p_{\trueq{b}}} {p^2_{b|\trueq{a}}} {p^2_{b|\trueq{b}}} {p_{a|\trueq{a}}} +  {p_{\trueq{a}}}{p_{\trueq{b}}} {p^2_{b|\trueq{b}}} {p^2_{b|\trueq{a}}} {p_{a|\trueq{b}}}
		\end{eqnarray*}
		which simplifies to
		\begin{eqnarray*}
			{p_{\trueq{a}}}{p_{\trueq{b}}} {p_{b|\trueq{a}}} {p_{b|\trueq{b}}} \cdot ({p_{a|\trueq{b}}}{p_{b|\trueq{a}}}{p_{b|\trueq{a}}} + {p_{a|\trueq{a}}}{p_{b|\trueq{b}}}{p_{b|\trueq{b}}}  
			- {p_{b|\trueq{b}}}{p_{a|\trueq{a}}}{p_{b|\trueq{a}}} - {p_{b|\trueq{a}}}{p_{a|\trueq{b}}} {p_{b|\trueq{b}}} ) \geq 0 .
		\end{eqnarray*}
		For the above inequality to hold, we should have:
		\begin{eqnarray*}
			{p_{a|\trueq{b}}}{p_{b|\trueq{a}}}{p_{b|\trueq{a}}} + {p_{a|\trueq{a}}}{p_{b|\trueq{b}}}{p_{b|\trueq{b}}}  
			- {p_{b|\trueq{b}}}{p_{a|\trueq{a}}}{p_{b|\trueq{a}}} - {p_{b|\trueq{a}}}{p_{a|\trueq{b}}} {p_{b|\trueq{b}}} \\ = 	{p_{b|\trueq{b}}}{p_{a|\trueq{a}}} ({p_{b|\trueq{b}}} - {p_{b|\trueq{a}}} ) - {p_{a|\trueq{b}}}{p_{b|\trueq{a}}} ({p_{b|\trueq{b}}} - {p_{b|\trueq{a}}})  \\= ({p_{b|\trueq{b}}}{p_{a|\trueq{a}}}-{p_{a|\trueq{b}}}{p_{b|\trueq{a}}}) ({p_{b|\trueq{b}}} - {p_{b|\trueq{a}}} ) \geq 0,
		\end{eqnarray*}
		which hold since ${p_{a|\trueq{a}}} \geq 1/2$ and ${p_{b|\trueq{b}}} \geq 1/2$.
		
	\end{proof}
	
	
	
	\begin{lemma}
		Under the assumption defined by \eqref{existanceoftruthful} and the conditional independence assumption, if ${p_{k|\trueq{k}}} \geq 1/2$ for $k \in \{a,b\}$, the signal joint distribution satisfies the following conditions:
		\begin{eqnarray} 
		{{p_{aab}}} \cdot  {{p_{ab}}} &\geq  {{p_{abb}}} \cdot  {{p_{bb}}} \label{property2}
		\end{eqnarray}
	\end{lemma} 
	
	
	
	\begin{proof}
		Similar to the previous lemma, for~\eqref{property2}, we can write:
		\begin{eqnarray*}
			({p^2_{a|\trueq{a}}P_{b|\trueq{a}}P_{\trueq{a}}}+ {p^2_{a|\trueq{b}}P_{b|\trueq{b}}P_{\trueq{b}}}) 
			\cdot ({p^2_{b|\trueq{a}} P_{\trueq{a}} + P^2_{b|\trueq{b}} P_{\trueq{b}} })  \\
			\geq ({p_{a|\trueq{a}} P^2_{b|\trueq{a}} P_{\trueq{a}}+ P_{a|\trueq{b}} P_{b|\trueq{b}}^2 P_{\trueq{b}}}) 
			\cdot ({p_{a|\trueq{a}} P_{b|\trueq{a}}  P_{\trueq{a}}+ P_{a|\trueq{b}} P_{b|\trueq{b}} P_{\trueq{b}}} ) .
		\end{eqnarray*}
		If we do the multiplications, we get:
		\begin{eqnarray*}
			{p_{\trueq{a}}P_{\trueq{b}}P_{b|\trueq{a}}P^2_{b|\trueq{b}}P^2_{a|\trueq{a}} }
			+ {p_{\trueq{a}}P_{\trueq{b}} P^2_{b|\trueq{a}} P_{b|\trueq{b}} P^2_{a|\trueq{b}}} 
			+ {p^2_{\trueq{a}} P^2_{a|\trueq{a}} P^3_{b|\trueq{a}} 
				+ P^2_{\trueq{b}} P^2_{a|\trueq{b}} P^3_{b|\trueq{b}}} \\
			\geq {p_{\trueq{a}}P_{\trueq{b}} P_{b|\trueq{b}} P_{a|\trueq{b}} P^2_{b|\trueq{a}} P_{a|\trueq{a}}} 
			+    {p_{\trueq{a}}P_{\trueq{b}} P_{a|\trueq{a}} P_{b|\trueq{a}} P^2_{b|\trueq{b}} P_{a|\trueq{b}}}  
			+ {p^2_{\trueq{a}} P^2_{a|\trueq{a}} P^3_{b|\trueq{a}}} +  { P^2_{\trueq{b}} P^2_{a|\trueq{b}} P^3_{b|\trueq{b}} }
		\end{eqnarray*}
		or
		\begin{eqnarray*}
			{p_{\trueq{a}} P_{\trueq{b}} P_{b|\trueq{b}} p_{b|\trueq{a}} (P_{b|\trueq{b}}P^2_{a|\trueq{a}}+ P_{b|\trueq{a}} P^2_{a|\trueq{b}}) } \geq 	{p_{\trueq{a}}P_{\trueq{b}} P_{b|\trueq{b}}P_{b|\trueq{a}}}  ( {p_{a|\trueq{a}} P_{b|\trueq{a}} P_{a|\trueq{b}} + P_{a|\trueq{b}} P_{a|\trueq{a}}P_{b|\trueq{b}}} )		
		\end{eqnarray*}
		By moving every term to the left side, we get:
		
		\begin{eqnarray*}
			{ P_{\trueq{a}} P_{\trueq{b}} P_{b|\trueq{b}} P_{b|\trueq{a}}} (  { P_{b|\trueq{b} }P^2_{a|\trueq{a}}+ P_{b|\trueq{a}} P^2_{a|\trueq{b}}} 
			- {p_{a|\trueq{a}}P_{b|\trueq{a}} P_{a|\trueq{b}} - P_{a|\trueq{b}} P_{a|\trueq{a}}P_{b|\trueq{b}}} ) \geq 0	
		\end{eqnarray*}
		which means we need to have:
		\begin{eqnarray*}
			{ P_{b|\trueq{b} }P^2_{a|\trueq{a}}+ P_{b|\trueq{a}} P^2_{a|\trueq{b}}} 
			- {p_{a|\trueq{a}}P_{b|\trueq{a}} P_{a|\trueq{b}} - P_{a|\trueq{b}} P_{a|\trueq{a}}P_{b|\trueq{b}}} = \\
			{		P_{b|\trueq{b}}P_{a|\trueq{a}} (P_{a|\trueq{a}}-P_{a|\trueq{b}})} 
			- {p_{b|\trueq{a}}P_{a|\trueq{b}} ( P_{a|\trueq{a}} - P_{a|\trueq{b}})} \\
			=  {(P_{b|\trueq{b}}P_{a|\trueq{a}} -  P_{b|\trueq{a}}P_{a|\trueq{b}})}  {(P_{a|\trueq{a}}-P_{a|\trueq{b}})} \geq 0,	
		\end{eqnarray*}
		which is true because $P_{a|\trueq{a}} \geq 1/2$ and $P_{b|\trueq{b}} \geq 1/2$.
	\end{proof}
	
	
	
	\begin{lemma}
		Under the assumption defined by \eqref{existanceoftruthful} and the conditional independence assumption, if ${p_{k|\trueq{k}}} \geq 1/2$ for $k \in \{a,b\}$, the signal joint distribution satisfies the following conditions:
		\begin{eqnarray}
		{{p_{aaab}}} \cdot  {{p_{bb}}}^2 &\geq  {{p_{abbb}}} \cdot  {{p_{ab}}}^2 \label{property3}
		\end{eqnarray}
	\end{lemma} 
	
	
	\begin{proof}
		To prove~\eqref{property3}, we first define the following:
		\begin{eqnarray*}
			\alpha = {p_{a|ab}}- {p_{a|\trueq{b}}} \text{ and }  \beta= {p_{b|ab}}- {p_{b|\trueq{a}}}. 
		\end{eqnarray*}
		If we observe another $a$, we will have that:
		\begin{eqnarray} \label{alpha}
		\alpha_{\text{new}} = \alpha \cdot \frac{\alpha+\beta+{p_{a|\trueq{b}}}}{\alpha+{p_{a|\trueq{b}}}}
		\end{eqnarray}
		If we observe another $b$, we get that:
		\begin{eqnarray} \label{beta}
		\beta_{\text{new}} = \beta \cdot \frac{\alpha+\beta+{p_{b|\trueq{a}}}}{\beta+{p_{b|\trueq{a}}}}.
		\end{eqnarray}
		Furthermore, we can write~\eqref{property3} as
		\begin{eqnarray*}
			\frac{{p_{aaab}}}{{p_{abbb}}} = \frac{{p_{aaab}}}{{p_{aabb}}} \cdot \frac{{p_{aabb}}}{{p_{bbbb}}} = \frac{{p_{a|aab}}}{{p_{b|aab}}} \cdot \frac{{p_{a|abb}}}{{p_{b|abb}}} \geq (\frac{{p_{ab}}}{{p_{bb}}})^2 = (\frac{{p_{a|b}}}{{p_{b|b}}})^2
		\end{eqnarray*}
		Based on~\eqref{alpha} and \eqref{beta}, write the above inequality as follows:
		\begin{eqnarray*}
			\frac{{p_{a|aab}}}{{p_{b|aab}}} \cdot \frac{{p_{a|abb}}}{{p_{b|abb}}}= \frac{ {p_{a|\trueq{b}}}+ \alpha \cdot  \frac{\alpha+\beta+{p_{a|\trueq{b}} }}{\alpha+{p_{a|\trueq{b}}}}}{ {p_{b|\trueq{a}}}+  \beta + \alpha - \alpha \cdot  \frac{\alpha+\beta+{p_{a|\trueq{b}} }}{\alpha+{p_{a|\trueq{b}}}}  } \cdot  \frac{{p_{a|\trueq{b}}}+\alpha+ \beta - \beta \cdot \frac{\alpha+\beta+{p_{b|\trueq{a}}}}{\beta+{p_{b|\trueq{a}}}} }{ {b|\trueq{a}} + \beta \cdot \frac{\alpha+\beta+{p_{b|\trueq{a}}}}{\beta+{p_{b|\trueq{a}}}}}  \\
			= \frac{(\alpha+{p_{a|\trueq{b}}})^2 + \alpha \beta}{(\alpha+{p_{a|\trueq{b}}})(\beta+{p_{b|\trueq{a}}})- \alpha \beta} \cdot \frac{(\alpha+{p_{a|\trueq{b}}})(\beta+{p_{b|\trueq{a}}})- \alpha \beta}{(\beta+{p_{b|\trueq{a}}})^2 + \alpha \beta} \\
			= \frac{(\alpha+{p_{a|\trueq{b}}})^2 + \alpha \beta}{(\beta+{p_{b|\trueq{a}}})^2 + \alpha \beta} \geq (\frac{\alpha+{p_{a|\trueq{b}}}- \frac{\alpha \beta}{\beta+{p_{a|\trueq{b}}}}}{\beta+{p_{b|\trueq{a}}} + \frac{\alpha \beta}{\beta+{p_{a|\trueq{b}}}}})^2 = (\frac{{p_{a|b}}}{{p_{b|b}}})^2
		\end{eqnarray*}
		which is true because by \eqref{property2}, $ \alpha+{p_{a|\trueq{b}}} \geq \beta+{p_{b|\trueq{a}}}$.
		
	\end{proof}
	
	\fi 
	
	
	





	\iffalse where $s_{ta}$ is the TA's signal and $y(.,.)$ is the perfect agreement reward function, i.e,
	\begin{align}  \label{spot-checkrewardcase}
	y(r_i,s_{ta}) = \left \lbrace
	\begin{array}{l l}
	1	& 	\text{if } r_i=s_{ta},   \\
	0  & 	\text{otherwise. } 
	\end{array}
	\right.
	\end{align}
	
	
	\fi


==> 2020-AAMAS_ Peer grading (arxiv)/numerical.tex <==
In this section, we use numerical experiments to quantify performance differences between the optimal DSIC RSS mechanism and the optimal DSIC ROS mechanism. For simplicity we consider $\conp{\firstsig}{\firstsig} = \conp{\secondsig}{\secondsig}$ (other settings yield qualitatively similar results but have more parameters over which to optimize).

First, we consider the case where each assignment is graded by three students,  as occurs in various practical peer grading systems \cite{wright2015mechanical,de2014crowdgrader}. Observe that TA workload can be computed given three quantities: $\frac{R}{c}$, the factor by which the reward exceeds the cost of effort; $\Prx{q}$, the prior over an assignment's true quality; and $\Prx{s|q}$, the prior over the grader's signal given a true quality. Given these quantities, let the \emph{scaled RSS workload} be the per-assignment TA workload required by the optimal DSIC RSS mechanism, expressed as a fraction of the per-assignment TA workload required by the optimal DSIC ROS mechanism. (Note that a scaled RSS workload of 1 means that RSS offers no benefits over ROS, and scaled RSS workloads approaching 0 correspond to  TA workloads under RSS that approach a 0\% fraction of those under ROS.) To investigate the scaled RSS workload empirically, we varied $\Prx{s|q}$ in 10\% increments from 0.6 (the signal gives little information about the true grade) to 1 (the signal perfectly identifies the true grade) and then set $\Prx{q}$ to {minimize} scaled RSS workload.\footnote{
    We already know that from Corollary~\ref{RSS saving2} that for every value of $\Prx{s|q}$ there exists a value of $\Prx{q}$ under which the scaled RSS workload is 1: the $\Prx{q}$ for which $\sum_q \Prx{s|q} \cdot \Prx{q}$ is uniform. Furthermore, note that for any fixed value of $\Prx{q}$, scaled RSS workload is unaffected by changes to $R/c$ (consult Equations \eqref{pstar}, \eqref{opt1}, and~\eqref{opt2}). However, Theorem~\ref{weaker} shows that as $\frac{R}{c}$ increases, a wider range of $\Prx{q}$ and $\Prx{s|q}$ distributions become feasible, allowing for smaller scaled RSS workloads. We thus focus on characterizing the smallest RSS workload that can be achieved for given values of $R/c$ and $\Prx{s|q}$.} 
The result is shown in Figure~\ref{fig:saving}. We make two key observations. First, scaled RSS workload starts out at 1 when rewards are similar to costs, but falls towards zero as $R/c$ increases. Second, holding $R/c$ constant, scaled RSS workload decreases as graders become more accurate (i.e., as $\Prx{s|q}$ approaches 1).
%Observe that when $\frac{c}{R}$ approaches 1/100, the saving percentage approaches 1. We start the graph at $\frac{c}{R}=\frac{1}{2}$ because that is the minimum ratio at which the optimal DSIC ROS and RSS mechanisms exist.

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.38 ]{images/saving1.pdf}
	\caption{Scaled RSS workload as a function of $R/c$ (on a log scale) and for different values of $\Prx{s|q}$, and for the value of $\Prx{q}$ that minimizes scaled RSS workload.}
	\label{fig:saving}
\end{figure}

Second, we investigate the relationship between the number of students grading each assignment and the scaled RSS workload. Observe that the optimal ROS mechanism gives rise to the same TA workload regardless of the number of students, while TA workload does change with the number of students under the optimal RSS mechanism. Figure~\ref{fig:prior} shows scaled RSS workload as a function of number of students for a setting with a moderately skewed prior distribution ($\Prx{q=a}=0.8$), relatively accurate graders ($\conp{\firstsig}{\firstsig}=0.9$), and a big gap between rewards and costs ($\frac{R}{c}={25}$).\footnote{Other values of these parameters yield different quantitative results but the same qualitative trends.} Overall, as the number of students grading each assignment increases, the scaled RSS workload increases (and hence the RSS mechanism offers less benefit over the ROS mechanism). To make this pattern more concrete, consider that when three students grade each assignment and follow their dominant strategies, the optimal ROS mechanism has a TA workload of $0.5$ while the optimal RSS mechanism has a TA workload of $0.18$ (a scaled RSS workload of 0.36); whereas, when $10$ students grade each assignment, the ROS workload remains at $0.5$ while the TA workload of the RSS mechanism increases to $0.23$ (for a scaled RSS workload of 0.47). 
%Note that the scaled RSS workload grows more and more slowly as the number of students increases; this is because in Equation~\eqref{Rss-saving}, as the number of students increases, $\joint{\Vec{\firstsig}}$ approaches 0. 
As the number of students grows, the scaled RSS workload approaches 0.58.
%Therefore, most of the saving is load is by cases where the probability of consulting the TA is the spot-checking probability of reporting signal $\secondsig$.

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.38]{images/n_students.pdf}
	\caption{Scaled RSS Workload as a function of number of students.}
	\label{fig:prior}
\end{figure}

% Next, we look into the TA workload of the optimal DSIC ROS and RSS mechanisms for different values $\Prx{s|q}$. In Figure~\ref{fig:noise}, we let $\joint{\firstsig}= 0.6$ and $\frac{c}{R}=\frac{1}{25}$, and vary $\conp{\firstsig}{\firstsig}$. This figure shows that when $\conp{\firstsig}{\firstsig}$ increases (i.e., as the students become more accurate graders), the total amounts of spot checking required by the optimal DSIC RSS and ROS mechanisms decrease, but the difference between the optimal DSIC RSS and ROS mechanisms decreases as well.



% \begin{figure}[t]
% 	\centering
% 	\includegraphics[scale=0.38 ]{images/ta_saving_noise.pdf}
% 	\caption{The TA workload of the optimal DSIC RSS and ROS mechanisms as a function of $\conp{\firstsig}{\firstsig}$.}
% 	\label{fig:noise}
% \end{figure}

==> 2020-AAMAS_ Peer grading (arxiv)/optimality.tex <==
We now characterize optimal DSIC mechanisms in both the ROS and RSS families. 

\subsection{Optimal DSIC ROS Mechanisms}

We begin by stating a result about ROS mechanisms from the literature.
%\hufu{The redundant sentence from the last section can be moved here, it seems.}
%\hufu{If we are not going to say anything about $x$ here, the following sentence seems not to belong here.}
Given a prior distribution $(\Pr[q])$ over the assignment's quality, the conditional signal distributions $\Prx{s|q}$, and the cost of the effort needed to examine the assignment and the reward $R$, there might be a minimum spot-checking probability~$\spotcheckpx$ (which is independent of~$n$, the number of students) that guarantees an ROS mechanism to be DSIC.
\begin{theorem} (Consequence of Lemma 1 in [\citealp{gao2016incentivizing}]) \label{uniform optimal} For any signal $\sig \in Q$, and any $c,R > 0$, if $ \joint{\secondsig \secondsig} - \joint{\firstsig \secondsig} \geq \frac{c}{R}$, a DSIC ROS mechanism spot checks a student with probability at least  
	% In the uniform spot checking mechanism, being truthful maximizes a student's utility if and only if the spot checking probability is at least:
	\begin{eqnarray}  \label{pstar}
	\spotcheckpx^* = \frac{\frac{c}{R}}{{\joint{\firstsig \firstsig}}+{\joint{\secondsig \secondsig}- \joint{\firstsig}}} = \frac{\frac{c}{R}}{{\joint{\secondsig \secondsig}}-{\joint{\firstsig \secondsig}}} ;
	\end{eqnarray}
	if 
	 $\joint{\secondsig \secondsig} - \joint{\firstsig \secondsig} < \frac{c}{R}$, there does not exist any DSIC ROS mechanism.
\end{theorem}

Recall that $\joint{\firstsig \secondsig}$ is the \emph{ex ante} probability that, when two signals $s_1$ and $s_2$ are drawn independently from $\Prx{s|q}$, $s_1 = \firstsig$ and $s_2 = \secondsig$. The assumption $\joint{\secondsig \secondsig} - \joint{\firstsig \secondsig} \geq \frac{c}{R}$ is necessary and sufficient to ensure that the ROS mechanism is DSIC if spot checks are performed with probability 1: a student who is always spot checked prefers to be truthful than to report either signal without effort. %Without this assumption, ROS mechanisms do not offer dominant strategies. %(Later, we will show that RSS mechanisms remain feasible in a broader range of settings.) 
We refer to $\spotcheckpx^*$ as the optimal DSIC ROS solution and the ROS mechanism that spot checks with probability~$\spotcheckpx^*$ as the optimal ROS mechanism. 

Equation~\eqref{pstar} demonstrates that TA workload of the optimal ROS mechanism falls as the reward--cost ratio $R/c$ increases. % and making $\spotcheckpx^*$ smaller .
However, both costs (effort required) and rewards (e.g., portion of a course grade devoted to performing peer review) are often fixed in practical peer grading scenarios. We thus take the approach of characterizing which (fixed) values of $R/c$ give rise to feasible spot-checking mechanisms and of investigating how spot-checking policies can be tuned to minimize TA workload.

\subsection{Optimal DSIC RSS Mechanisms}

We begin by defining a class of mechanisms and then go on to prove our first main result: that a mechanism from this class minimizes TA workload across all DSIC RSS mechanisms. 

\begin{definition}[PRSS Mechanism]
A \emph{Personal-Report-Sensitive Spot-checking mechanism}, or \emph{PRSS mechanism}, spot checks each student with a probability that only depends on the student's own report.
\end{definition}
In PRSS mechanisms, the functions $\spotcheckpx_\firstsig$ and $\spotcheckpx_\secondsig$ are constant, i.e., for $ \forall j,j' \in \{0,\dots,n\}$ and $j \neq j'$, $\spotcheckp{\firstsig}{j} = \spotcheckp{\firstsig}{j'}$ and $\spotcheckp{\secondsig}{j} = \spotcheckp{\secondsig}{j'}$.  A remarkable feature of PRSS mechanisms is that, if $\spotcheckpx_{\firstsig}(k) \neq \spotcheckpx_{\secondsig}(k)$ for some~$k$, the TA's input is sometimes ``wasted'', in the sense that it is not used to spot check every student.  To see this, say if $\spotcheckpx_{\secondsig}(k) > \spotcheckpx_{\firstsig}(k)$, then the mechanism should consult the TA with probability $\spotcheckpx_{\secondsig}(k)$ but spot checks a student reporting~$\firstsig$ with probability only~$\spotcheckpx_{\firstsig}(k)$.

% , i.e., the spot-checking probability for each student only depends on whether their reported signal is $\firstsig$ or $\secondsig$.

Our first result is a characterization of the optimal DSIC RSS mechanism.  We show that this optimum is achieved by a PRSS mechanism with appropriate spot-checking probabilities. We also characterize the necessary and sufficient condition for the existence of DSIC RSS mechanisms. Later we show that this condition is weaker than the one for DSIC ROS mechanisms in Theorem~\ref{weaker}.


\begin{theorem} \label{main}
	\label{thm:opt-RSS}
	For any signal $\sig_i \in Q$, and any $c,R > 0$, if  $\sigcond{\firstsig}{\firstsig} - \joint{\firstsig} \geq \frac{c}{R}$, 
	a PRSS mechanism with the following spot-checking probabilities is the DSIC spot-checking mechanism that minimizes the TA workload among all other DSIC spot-checking mechanisms:
	\begin{align}
	\spotcheckp{\firstsig}{k} &=  \frac{  \frac{c}{R} }{\sigcond{\secondsig}{\secondsig} - \joint{\secondsig}} \ \ \ \forall k \in \{1,\dots,n\}   \label{opt1} \\
	\spotcheckp{\secondsig}{k} &=  \frac{  \frac{c}{R}}{\sigcond{\firstsig}{\firstsig} - \joint{\firstsig}} \ \ \ \forall k \in \{0,\dots,n-1\}; \label{opt2}
	\end{align}
	if
	$\sigcond{\firstsig}{\firstsig} - \joint{\firstsig} < \frac{c}{R} $,
	there does not exist any DSIC spot-checking mechanism.
	% minimize the expected amount of any RSS mechanism assuming that everyone is truthful and under the DSIC constraints.
\end{theorem}


This result is nontrivial.  Recall that an RSS mechanism has the power to vary the spot-checking probabilities for each student based on the reports of all other students, and such side information conceivably could help reduce the TA workload while maintaining the students' incentives.  This turns out not to be the case.  One immediate consequence of Theorem~\ref{thm:opt-RSS} is that the TA workload \emph{increases} with the number of students grading each assignment.
%\hufu{Restated the theorem and added the paragraph above.  Please check if it's ok.  Feel free to briefly explain the proof idea.}
 
The proof consists of two steps.  In Step~$1$, we reason about a convex optimization problem that minimizes the workload but relaxes all of the DSIC constraints except those that incentivize the truthful strategy when all other students make no effort. We show that the intersection point of the non-trivial constraints in this optimization problem is locally optimal, and hence, also, the global optimal of the defined optimization problem.  Then, in Step~$2$, we show that this solution in fact gives rise to a DSIC RSS mechanism.  Since it is an optimal solution with most DSIC constraints relaxed, it is also optimal when one enforces all constraints.

% observe that the obtained optimal solution does not depend on the value of $k$: i.e., that it results in a PRSS mechanism. We use this independence to argue that the obtained optimal solution indeed satisfies all the DSIC constraints because the utility of each student does not depend on what others do. %Therefore, an RSS mechanism that uses the values defined by~\eqref{opt1} and \eqref{opt2} as its spot-checking functions is the optimal DSIC mechanism.   

\begin{proof}
%\vspace{0.03in}
	\noindent
	\textbf{Step~1.} In a DSIC mechanism, fixing a student~$i$, if all students other than~$i$ report a signal without expending effort, $i$ should be incentivized to be truthful, i.e., to invest effort and to report the signal observed.  Suppose $k$ other students report~$\firstsig$: then, the utility of student~$i$ reporting signal~$\firstsig$ without investing effort is $R \cdot \Prx{\sigta = \firstsig} \cdot \spotcheckp{\firstsig}{k+1}$, whereas her utility for being truthful is 
	\begin{multline*}
	R \cdot (	\Prx{\sig_i=\firstsig} \cdot \Prx
		%[\sigta \sim \conp{\sig}{s_i=a}]
		{\sigta = \firstsig \given s_i = \firstsig}  \spotcheckp{\firstsig}{k+1} \\
	+ 	\Prx{\sig_i=\secondsig} \cdot \Prx 
	%[\sigta \sim \conp{\sig}{s_i = b}]
	{\sigta = \secondsig \given s_i = \secondsig} \spotcheckp{\secondsig}{k} ) - c.
	\end{multline*}
We therefore should have that, for $k \in \{0, \ldots, n - 1\}$,
	\begin{multline}
	\Prx{\sig_i=\firstsig} \cdot \Prx
	%[\sigta \sim \conp{\sig}{s_i=a}]
	{\sigta = \firstsig \given s_i = \firstsig}  \spotcheckp{\firstsig}{k+1}  \\
	+ \Prx{\sig_i=\secondsig} \cdot \Prx
	%[\sigta \sim \conp{\sig}{s_i = b}]
	{\sigta = \secondsig \given s_i = \secondsig} \spotcheckp{\secondsig}{k} \\
	- \Prx{\sigta = \firstsig} \spotcheckp{\firstsig}{k+1}	\geq  \frac{c}{R}.
	\label{eq:ica-lazy-opponents}
	\end{multline}
	Similarly we should have for $k \in \{0, \ldots, n - 1\}$ that
	\begin{multline}
		\Prx{\sig_i=\firstsig} \cdot \Prx{\sigta = \firstsig \given s_i = \firstsig}  \spotcheckp{\firstsig}{k+1} \\
	+ 	\Prx{\sig_i=\secondsig} \cdot \Prx{\sigta = \secondsig \given s_i = \secondsig} \spotcheckp{\secondsig}{k}  \\
	 - \Prx{\sigta = \secondsig} \spotcheckp{\secondsig}{k}	\geq  \frac{c}{R}.
		\label{eq:icb-lazy-opponents}
	\end{multline}
	
	Simplifying \eqref{eq:ica-lazy-opponents} and \eqref{eq:icb-lazy-opponents}, we have 
%	--\eqref{eq:misreport-a-b} further, we get the following four expressions:
		\begin{eqnarray}
	-{\joint{\firstsig \secondsig }}     \spotcheckp{\firstsig}{k+1} + {\joint{\secondsig \secondsig }}    \spotcheckp{\secondsig }{k}  \geq \frac{c}{R}. \label{eq:ica-lazy-opponents-simplified} \\
	{\joint{\firstsig \firstsig }}     \spotcheckp{\firstsig}{k+1} - {\joint{\firstsig \secondsig }}    \spotcheckp{\secondsig }{k}  \geq \frac{c}{R}. \label{eq:icb-lazy-opponents-simplified}
	\end{eqnarray}

	% Accordingly, \klb{accordingly: what is this referring to? The fact that there are two signals?}
	
	Consider minimizing the TA workload subject to \eqref{eq:ica-lazy-opponents-simplified} and~\eqref{eq:icb-lazy-opponents-simplified}: 
	\begin{multline*}
		\min_{\substack{\spotcheckpx_{\firstsig}, \spotcheckpx_{\secondsig}}}  \sum_{t \in Q} \trueqp{t} \sum_{j = 0}^n \binom{n}{j} (\conp{\firstsig}{t})^j \\\cdot (\conp{\secondsig}{t})^{n - j} \max\{\spotcheckp{\firstsig}{j}, \spotcheckp{\secondsig}{j}\}. % \label{obj0}  
	\end{multline*}
	with $0 \leq \spotcheckpx_{\firstsig}(k), \spotcheckpx_{\secondsig}(k) \leq 1$ for all $k \in \{0, \cdots, n\}$.  The value of this optimization problem is an upper bound to the workload of any DSIC mechanism, since it relaxed all DSIC constraints except \eqref{eq:ica-lazy-opponents} and \eqref{eq:icb-lazy-opponents}.  Note also that the objective function is convex in the variables, due to the presence of the $\max$ functions, and its feasible region is a convex polytope since all constraints are linear.  There are $2n$ variables: $x_{\secondsig}(0), x_{\firstsig}(1), x_{\secondsig}(1), x_{\firstsig}(2), \ldots, x_{\firstsig}(n-1), x_{\secondsig}(n-1), x_{\firstsig}(n)$.  (Note that $x_{\firstsig}(0)$ and $x_{\secondsig}(n)$ are zero.)  These variables can be grouped into $n$~pairs, with $x_{\secondsig}(k)$ and $x_{\firstsig}(k+1)$ as a pair for each~$k$.  Each pair is subject to a pair of constraints from \eqref{eq:ica-lazy-opponents-simplified} and~\eqref{eq:icb-lazy-opponents-simplified} with the corresponding~$k$, and there is no constraint governing variables from different pairs.  This means the optimization problem is separated into $n$~subproblems, one for each pair of variables.  We now claim that the optimal solution for each subproblem is given by forcing \eqref{eq:ica-lazy-opponents-simplified} and~\eqref{eq:icb-lazy-opponents-simplified} to be tight, which gives us the following expressions:
	\begin{align}
	 \spotcheckp{\firstsig}{k} &=  \frac{c}{R} \cdot \frac{  \joint{\secondsig}}{\joint{\firstsig \firstsig}\joint{\secondsig \secondsig }-(\joint{ \firstsig \secondsig})^2} \ \ \ \forall k \in \{1,\dots,n\} \label{long-opt1} \\
	\spotcheckp{\secondsig}{k} &=  \frac{c}{R}\cdot \frac{  \joint{\firstsig }}{\joint{\firstsig \firstsig }\joint{\secondsig \secondsig }-(\joint{\firstsig\secondsig })^2} \ \ \ \forall k \in \{0,\dots,n-1\}; \label{long-opt2}     
	\end{align}
	Simplifying \eqref{long-opt2}, we get
	\begin{align*}
	 \spotcheckp{\secondsig}{k} &=  \frac{c}{R}\cdot \frac{\joint{\firstsig}}{\joint{\firstsig \firstsig }\joint{\secondsig \secondsig }-(\joint{\firstsig\secondsig })^2} = \frac{c}{R}\cdot \frac{\joint{\firstsig}}{\joint{\firstsig \firstsig }\joint{\secondsig \secondsig } - \joint{\firstsig\secondsig } (\joint{\firstsig}- \joint{ \firstsig \firstsig})} \\
	   &= \frac{c}{R}\cdot \frac{\joint{\firstsig}}{\joint{\firstsig \firstsig }\joint{\secondsig}-\joint{\firstsig}\joint{\firstsig\secondsig }} = \frac{c}{R}\cdot \frac{\joint{\firstsig}}{\joint{\firstsig \firstsig }(1-\joint{\firstsig})-\joint{\firstsig}\joint{\firstsig\secondsig }}  \\
	   &=  \frac{\frac{c}{R}}{\frac{\joint{\firstsig \firstsig }}{\joint{\firstsig }} - \joint{\firstsig}} 
	   = \frac{\frac{c}{R}}{\sigcond{\firstsig}{\firstsig} - \joint{\firstsig}} ,
	\end{align*}
	which is the expression in \eqref{opt2}. We get the expression in ~\eqref{opt1} by simplifying \eqref{long-opt1}, similarly. 
	
	We first check that these solutions are feasible: we have that $\joint{\firstsig} > \joint{\secondsig}$ in~\eqref{long-opt1} and~\eqref{long-opt2}, therefore, if $\sigcond{\firstsig}{\firstsig} - \joint{\firstsig} \geq \frac{c}{R}$, the spot-checking probabilities are indeed between $0$ and~$1$.
	To see that these solutions are optimal, we invoke the convexity of the problem, which means we only need to argue that the solutions are locally optimal.  At the point where \eqref{eq:ica-lazy-opponents-simplified} and~\eqref{eq:icb-lazy-opponents-simplified} are tight for a given~$k$, increasing $x_{\firstsig}(k+1)$ forces $x_{\secondsig}(k)$ to increase, and vice versa, in order for the pair to keep being feasible --- this is a consequence of the coefficients' signs in \eqref{eq:ica-lazy-opponents-simplified} and~\eqref{eq:icb-lazy-opponents-simplified} --- but it is not feasible to decrease both variables. Therefore the only local move within the feasible region is to increase both variables.  However, both variables have positive coefficients in the objective function.  Therefore the solution in \eqref{opt1} and~\eqref{opt2} is both locally optimal and globally optimal for our convex program.
	 
	 We note that if $\sigcond{\firstsig}{\firstsig} - \joint{\firstsig} < \frac{c}{R} $, to make sure that Constraints \eqref{eq:ica-lazy-opponents-simplified} and~\eqref{eq:icb-lazy-opponents-simplified} are all satisfied for $k \in \{0, \ldots, n - 1\}$, at least one of $x_{\secondsig}(k)$ or $x_{\firstsig}(k+1)$ has to be strictly greater than one. This is also a consequence of the coefficients' signs in \eqref{eq:ica-lazy-opponents-simplified} and~\eqref{eq:icb-lazy-opponents-simplified}. However, $0 \leq \spotcheckpx_{\firstsig}(k), \spotcheckpx_{\secondsig}(k) \leq 1$ for all $k \in \{0, \cdots, n - 1\}$. Therefore, there does not exist any feasible DSIC RSS mechanism.
	 
	 
 % In this optimization problem (which we call the ``RSS convex optimization problem''), 
 % \klb{This seems to be referred to only in one place. Does it really need a name?}\hedayat{I also refer to it in the proof of the last theorem}the objective function is convex, because it is a non-negative weighted sum of a set of piece-wise linear convex functions ($\max\{\spotcheckp{a}{k}, \spotcheckp{b}{k}\}$, for $k \in \{0, \ldots, n \}$).\klb{Is it enough just to state this?} \hedayat{added an argument for convexity} Furthermore, for each $k \in \{0, \ldots, n - 1\}$, the decision variables within each pair of constraints do not appear in any other similarly \klb{what does it mean "similarly"?}defined pairs of constraints. Since the sign of each decision variable in each pair switches from one constraint to another, at the intersection of each pair, the only way to preserve feasibility is to increase both of the decision variables together. However, this would only increase the objective value because every objective coefficient is positive. Therefore, there is no local move from the intersections of the pairs of the constraints which would result in an improvement in the objective value. Since the optimization problem is convex, local optima are also globally optimal; hence, such intersections of pairs of constraints, if feasible, would be the optimal solution. By Assumptions~\ref{assn:spot-check-prob-1} and \ref{assn:spot-check-prob-2}, $\joint{bb} - \joint{ab} \geq c  $ and $\joint{aa} \geq \joint{ab}$, which means the obtained values satisfy $0 \leq \spotcheckpx_{a}, \spotcheckpx_{b} \leq 1$, and hence are feasible. Since every pair of constraints has the same set of coefficients \klb{a pair has one coefficient?} \hedayat{changed it to set of coefficients}but different decision variables,  every intersection has the form defined by~\eqref{opt1} and~\eqref{opt2}. Hence, the resulting optimal spot-checking functions are fixed and we indeed have a PRSS mechanism.

	\vspace{0.03in}
	\noindent
	\textbf{Step~2.} We now show that the spot-checking probabilities given in \eqref{opt1} and~\eqref{opt2} in fact give rise to a DSIC mechanism.  We only need to check the validity of the DSIC constraints not included in the convex program above.
	
	% So far, our calculations have only taken into account the case in which all students other than~$i$ report a signal without spending effort. To complete the proof, we must show that the obtained optimal solution is a DSIC mechanism: i.e., for any strategies that the other students choose, student $i$'s utility-maximizing strategy is truthful. 
	
	We first check the condition that a student having spent the effort to get a signal should be incentivized to report the observation faithfully.   % Furthermore, student $i$ should prefer to report her observed signal instead of misreporting. Therefore, we should also have that, 
	We need for $k \in \{0, \ldots, n - 1\}$,
	\begin{multline}
		 \Prx{\sigta = \firstsig \given s_i = \firstsig}  \spotcheckp{\firstsig}{k+1}  \\
		 \geq 
	 \Prx{\sigta = \secondsig \given s_i = \firstsig} \spotcheckp{\secondsig}{k}, 
		% \label{eq:misreport-b-a}
	\end{multline}
	and 
	\begin{multline}
		 \Prx{\sigta = \secondsig \given s_i = \secondsig}  \spotcheckp{\secondsig}{k}  \\
		 \geq 
	 \Prx{\sigta = \firstsig \given s_i = \secondsig} \spotcheckp{\firstsig}{k+1},
		% \label{eq:misreport-a-b}
	\end{multline}
	which simplify to
\begin{eqnarray}
	{\joint{\firstsig \firstsig}}     \spotcheckp{\firstsig}{k+1} - {\joint{\firstsig \secondsig }}    \spotcheckp{\secondsig}{k}  \geq 0.  \label{eq:misreport-b-a-simplified}\\
	-{\joint{\firstsig \secondsig }}     \spotcheckp{\firstsig}{k+1} + {\joint{\secondsig \secondsig }}    \spotcheckp{\secondsig}{k}   \geq 0. \label{eq:misreport-a-b-simplified}
	\end{eqnarray}
	Note that \eqref{eq:misreport-b-a-simplified} and \eqref{eq:misreport-a-b-simplified} are in fact implied by \eqref{eq:ica-lazy-opponents-simplified} and~\eqref{eq:icb-lazy-opponents-simplified}.  
	% This means that if the spot-checking functions are such that student $i$ prefers to expend effort, she would also prefer to report her observed signal to the mechanism instead of misreporting. We note that this property crucially depends on the fact that there are only two possible signals.  
	
	For the other DSIC constraints that concern a student's utility when some other students may spend effort to observe a signal, note that the spot-checking probabilities given by \eqref{opt1} and~\eqref{opt2} are independent of~$k$, i.e., they are independent from what the other students report, and therefore the corresponding mechanism is PRSS.  In such a mechanism, a student's utility is independent from the other students' strategies.  If the truthful strategy maximizes a student's utility when no other student spends any effort, it still does when other students spend effort.  Therefore the mechanism obtained from Step~$1$ is indeed DSIC, and this completes the proof.
	% Based on the solution obtained in Step 1, for $k \in \{0, \ldots, n - 1\}$, since $\spotcheckp{a}{k} \leq \spotcheckp{b}{k}$, the probability that the assignment is spot checked is $\max\{\spotcheckp{a}{k}, \spotcheckp{b}{k}\}=\spotcheckp{b}{k}$.  In this case, once the assignment is spot checked, we spot check the students who reported signals $\firstsig$ and $\secondsig$ with probabilities $\frac{\spotcheckp{a}{k}}{\spotcheckp{b}{k}}$ and $1$, respectively. When $k=n$, we spot check the assingment and thus, each student, with probability $\spotcheckp{a}{k}$. This way we can ensure that the spot-checking functions for each individual student follows those defined by~\eqref{opt1} and~\eqref{opt2}. This means that students' spot-checking probabilities (and therefore their utilities) are independent of what others do: the mechanism is PRSS. Based on the RSS convex optimization program, the spot-checking functions defined by~\eqref{opt1} and \eqref{opt2} ensure that truthfulness is a utility-maximizing strategy mechanism while the constraints that guarantee dominant strategy truthfulness have exactly the same form as~\eqref{eq:ica-lazy-opponents}--\eqref{eq:icb-lazy-opponents}.
	\end{proof}


%We note that Equation~\eqref{pstar} implies that one can reduce the TA workload of the optimal ROS mechanism by increasing the reward $R$ and making $\spotcheckpx^*$ smaller . However, arbitrarily scaling up the rewards does not make sense in many practical peer grading scenarios. Our approach, i.e., fixing the reward to be a constant, making some feasibility assumptions, and minimizing the TA workload accordingly---attempts to reason about how TA workload can be reduced in such settings. 

 The following theorem shows that for a given set of input distributions, while the optimal DSIC RSS mechanism might be feasible, there might not exist any DSIC ROS mechanism.

%\hufu{The corollary needs to be more specific.  from the statement one can't tell whether are situations when one holds and the other doesn't.  It could be ``whenever there is a DSIC ROS mechanism, there is a DSIC RSS mechanism; and when blah, DSIC RSS exists and the other doesn't.''  Also a short discussion of this should precede the statement.}
\begin{theorem} \label{weaker}
For any signal $s \in Q$, and any $c,R > 0$, whenever there is a DSIC ROS mechanism, there is a DSIC RSS mechanism; however, when $\joint{\firstsig} > \joint{\secondsig}$, there exist $c,R > 0$ for which $\joint{\secondsig\secondsig} - \joint{\firstsig\secondsig} < \frac{c}{R} \leq \sigcond{\firstsig}{\firstsig} - \joint{\firstsig}  $, i.e., the optimal DSIC RSS mechanism exists while DSIC ROS mechanisms do not. 
\end{theorem}

\begin{proof}
	 By Theorem~\ref{main}, we know that for any signal $\sig_i \in Q$ and any $c,R > 0$, if $\frac{c}{R} \geq \sigcond{\firstsig}{\firstsig} - \joint{\firstsig} = \frac{\joint{\firstsig \firstsig }\joint{\secondsig \secondsig }-(\joint{\firstsig\secondsig })^2}{\joint{\firstsig}}$, then the optimal DSIC RSS mechanism exists. Therefore, we only need to show that  $\frac{\joint{\firstsig \firstsig }\joint{\secondsig \secondsig }-(\joint{\firstsig\secondsig })^2}{\joint{\firstsig}}  > \joint{\secondsig\secondsig} - \joint{\firstsig\secondsig} $, i.e., there is a gap between these expressions. We can write
\begin{align*}
	\joint{\firstsig \firstsig} \cdot \joint{\secondsig \secondsig} - \joint{\firstsig\secondsig}^2  &>   \joint{\firstsig \firstsig} \cdot \joint{\secondsig \secondsig} - \joint{\firstsig\secondsig}^2 - \joint{\firstsig\secondsig} \cdot ( \joint{\firstsig \firstsig}- \joint{\secondsig \secondsig} ) \\
	&= (\joint{\firstsig \firstsig} + \joint{\firstsig \secondsig}) (\joint{\secondsig \secondsig} - \joint{\firstsig \secondsig}) = \joint{\firstsig} \cdot (\joint{\secondsig \secondsig} - \joint{\firstsig \secondsig}),
	\end{align*}	
	where the first inequality is dues to the fact that $ \joint{\firstsig \firstsig} > \joint{\secondsig \secondsig} $. %This means that for any signal $s \in Q$:
%	\begin{align*}
%	    \frac{\joint{\firstsig \firstsig }\joint{\secondsig \secondsig }-(\joint{\firstsig\secondsig })^2}{\joint{\firstsig}} &= \sigcond{\firstsig}{\firstsig} - \joint{\firstsig} <  \joint{\secondsig \secondsig} - \joint{\firstsig \secondsig} 
%	\end{align*} 
	
	
\end{proof}











	\iffalse
	First, we define and solve an optimization problem that minimizes the TA workload of any spot-checking mechanism, assuming that all students are truthful subject to a subset of the DSIC constraints that imply that truthfulness is the utility maximizing strategy when others make no effort. Then we show that the optimal solution to this problem satisfies all the DSIC constraints, and hence results in the optimal DSIC RSS mechanism. For any student $i$ we have:
	\begin{multline}
	\min_{\substack{\spotcheckpx_{\firstsig}, \spotcheckpx_{\secondsig}}}    \sum_{t \in Q} \trueqp{t} \sum_{j = 0}^n \binom{n}{j} (\conp{\firstsig}{t})^j \\\cdot(\conp{\secondsig}{t})^{n - j} \max\{\spotcheckp{\firstsig}{j}, \spotcheckp{\secondsig}{j}\} \label{obj0}  
	\end{multline}
	subject to:	
	\begin{align}
	& \Ex[s_i]{   \Ex[\sigta \sim \conp{\sig}{s_i=\firstsig}]{Y(\firstsig, \sigta)}  \spotcheckp{\firstsig}{k+\mathbbm{1}_{s_i=\firstsig}}} \label{firstgroup} \\
	&-  \Ex[\sigta \sim \joint{\sig}]{Y(\firstsig, \sigta)} \spotcheckp{\firstsig}{k+1} \geq \frac{c}{R}, \ \forall k \in \{0,\dots,n-1\} \nonumber \\
	& \Ex[s_i]{ \Ex[\sigta \sim \conp{\sig}{s_i=\firstsig}]{Y(\firstsig, \sigta)} \spotcheckp{\firstsig}{k+\mathbbm{1}_{s_i=\firstsig}}} \label{firstgroup1} \\
	&-  \Ex[\sigta \sim \joint{\sig}]{Y(\secondsig, \sigta)} \spotcheckp{\secondsig}{k}  \geq \frac{c}{R}, \ \forall k \in \{0,\dots,n-1\}  \nonumber  \\
	&   \Ex[\sigta \sim \conp{\sig}{s_i=\firstsig}]{Y(\firstsig, \sigta)}  \spotcheckp{\firstsig}{k+1} \label{second group}\\
	&\geq   \Ex[\sigta \sim \conp{\sig}{s_i=\firstsig}]{Y(\firstsig, \sigta)} \spotcheckp{\secondsig}{k}, \ \forall k \in \{0,\dots,n-1\} \nonumber \\
	&   \spotcheckp{\secondsig}{k} \Ex[\sigta \sim \conp{\sig}{s_i=\secondsig}]{Y(\secondsig, \sigta)} \label{second group1}\\
	&\geq   \Ex[\sigta \sim \conp{\sig}{s_i=\secondsig}]{Y(\firstsig, \sigta)} \spotcheckp{\firstsig}{k+1}, \ \forall k \in \{0,\dots,n-1\} \nonumber \\
	& 0 \leq \spotcheckp{\firstsig}{k}, \spotcheckp{\secondsig}{k} \leq 1. \  \forall k \in \{0,\dots,n\}  \label{third group}
	\end{align}	
	
	In this optimization problem (which we call the ``RSS convex optimization problem''), the objective function defined by~\eqref{obj0} is convex and calculates the TA workload assuming that all the students are truthful (see Def.~\ref{TAworkload def}). Constraints \eqref{firstgroup} and \eqref{firstgroup1} ensure that each student would achieve higher utility by being truthful than by reporting an arbitrary signal, when every other student does not invest effort. Constraints \eqref{second group} and \eqref{second group1} ensure that each student gets more utility by reporting their observed signal (rather than misreporting), when every other student does not invest effort. 
	
	Since %we assume that 
	every student except $i$ does not invest effort, for any $k \in \{0,\dots,n-1\}$, we can simplify Constraint \eqref{firstgroup} as:
	\begin{align}
	& \scalebox{0.89}[1]{$\joint{\firstsig}       \left(  \Pr(\sigta=\firstsig|s=\firstsig)    Y(\firstsig,\firstsig)  + \Pr(\sigta=\secondsig|s=\firstsig)    Y(\firstsig,\secondsig) \right) \spotcheckp{\firstsig}{k+1} $} \nonumber \\
	& \ \scalebox{0.89}[1]{$ + \joint{\secondsig}         \left(\Pr(\sigta=\secondsig|s=\firstsig)    Y(\firstsig,\secondsig)  + \Pr(\sigta=\secondsig|s=\secondsig)    Y(\secondsig,\secondsig) \right)  \spotcheckp{\secondsig}{k} $} \nonumber\\
	& ~~~~~~~~~~~~~~~~~~~~~~~\scalebox{0.89}[1]{$-   \left(\joint{\firstsig}    Y(\firstsig,\firstsig) + \joint{\secondsig}    Y(\firstsig,\secondsig) \right) \spotcheckp{\firstsig}{k+1} \geq \frac{c}{R} $} . \label{above}
	\end{align}
	Using the definition of $Y(\firstsig,\sigta)$, \eqref{above} simplifies to:
	\begin{eqnarray}
	-{\joint{\firstsig \secondsig }}     \spotcheckp{\firstsig}{k+1} + {\joint{\secondsig \secondsig }}    \spotcheckp{\secondsig}{k}  \geq \frac{c}{R}. \label{11}
	\end{eqnarray} 
	Similarly, for Constraints~\eqref{firstgroup1}, ~\eqref{second group}, and \eqref{second group1}, for any $k \in \{0,\dots,n-1\}$, we get:
	\begin{eqnarray}
	{\joint{\firstsig \firstsig}}     \spotcheckp{\firstsig}{k+1} - {\joint{\firstsig \secondsig }}    \spotcheckp{\secondsig}{k}  \geq \frac{c}{R}. \label{12} \\
	{\joint{\firstsig \firstsig }}     \spotcheckp{\firstsig }{k+1} - {\joint{\firstsig \secondsig}}    \spotcheckp{\secondsig}{k}  \geq 0.  \label{13}\\
	-{\joint{\firstsig \secondsig }}     \spotcheckp{\firstsig}{k+1} + {\joint{\secondsig \secondsig }}    \spotcheckp{\secondsig}{k}   \geq 0. \label{14}
	\end{eqnarray}
	Inequalities~\eqref{11}--\eqref{14} show that  Constraints~\eqref{second group}, and \eqref{second group1} are implied by Constraints~\eqref{firstgroup} and~\eqref{firstgroup1} and can be removed from the optimization problem without changing the optimal solution. Once Constraints~\eqref{firstgroup} and~\eqref{firstgroup1} are removed, for any $k \in \{0,\dots,n-1\}$, the decision variables within each pair of constraints defined by \eqref{11} and \eqref{12} (i.e., one that describes student $i$ reporting $\firstsig$ with no effort and the other describing $i$ reporting $\secondsig$ with no effort) do not appear in any other similarly defined pairs of constraints. Furthermore, in each pair, since the sign of each decision variable switches from one pair to another, at the intersection of each pair, the only way to preserve feasibility is to increase both of the decision variables together. However, this would only increase the objective value because every objective coefficient is positive. Therefore, there is no local move from the intersections of the pairs of the constraints which would result in an improvement in the objective value. Since the optimization problem is convex, local optima are also globally optimal; hence, such intersections of pairs of constraints, if feasible, would be the optimal solution. However, by Assumptions~\ref{assn:spot-check-prob-1} and \ref{assn:spot-check-prob-2}, $\joint{\secondsig \secondsig} - \joint{ \firstsig \secondsig} \geq c  $ and $\joint{\firstsig \firstsig} \geq \joint{ \firstsig \secondsig}$, which means the obtained values satisfy Constraint \eqref{third group} and hence are feasible. Notice that any pair of constraints have the same coefficient but different decision variables. Therefore, each intersection has the form defined by~\eqref{opt1} and~\eqref{opt2}.   
	
	\klb{Gets a bit informal from this point on.}
	To complete the proof, we show that the obtained optimal solution indeed satisfies all the DSIC constraints. The spot-checking probabilities defined by~\eqref{opt1} and~\eqref{opt2} are independent from $k$. When the reported signals for an assignment include at least one signal $\secondsig$ (i.e., we spot check the assignment with probability $\max\{\spotcheckpx^a,\spotcheckpx^b\}=\spotcheckpx^b$, since $\joint{a} \geq \joint{b}$), if we spot check the students who reported signal $\firstsig$ and $\secondsig$, with probabilities $\frac{\spotcheckpx^a}{\spotcheckpx^b}$ and $\spotcheckpx^b$, respectively, we ensure that the spot-checking probabilities for such individual students are $\spotcheckpx^a$ and $\spotcheckpx^b$. This means that their spot-checking probabilities (and therefore their utilities) are not dependent on what others do. As a result, an RSS mechanism in which the spot-checking probabilities are defined by~\eqref{opt1} and \eqref{opt2} can be considered as a single-agent report-sensitive mechanism, where there is only one student grading the assignment. Based on the RSS convex optimization program, the spot-checking probabilities defined by~\eqref{opt1} and \eqref{opt2} result in truthfulness being the utility maximizing strategy in the single-agent report-sensitive mechanism because $(i)$ there is only one strategic grader and $(ii)$ the constraints that guarantee the dominant strategy truthfulness have exactly the same form as~\eqref{firstgroup}-\eqref{third group} when $n=1$. 
	
	\fi

